HyInv Technical Report

Inverse folding designs amino-acid sequences for a given protein backbone, and screening needs many candidates that are both diverse and well folded. We present HyInv, a 1.96-million-parameter backbone-conditioned graph network with an encoder-decoder architecture, trained by Hyra 2.0, the research agent developed by our team: pretrained with random-order autoregressive sequence modeling, followed by structure-reward reinforcement learning. At inference, a grouped draft-and-rewrite sampler that uses separate draft and rewrite temperatures improves refolding TM-score at matched diversity. An optimized implementation with BF16 numerics designs 128 sequences for a 402-residue backbone in 50.6 ms on a single NVIDIA H20 GPU, about 52 times faster than the reference sampler, and an exact FP32 path that returns the reference sequences is 8.7 times faster. Across five benchmark datasets and seven dataset-predictor combinations, HyInv reaches a higher average scTM than all ten external baselines at comparable or higher sequence diversity, with large margins over ProteinMPNN and ProteinZero V2. The same default setting supports de novo backbones, pocket-constrained libraries, enzyme redesign with the catalytic site kept, and loop redesign. We have released our code and model at https://github.com/Tencent-Hunyuan/Hyra-results/tree/main/AI4Science/hyinv.

==> texmf/tex/generic/tracklang/tracklang.tex <==
%%
%% This is file `tracklang.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% tracklang.dtx  (with options: `tracklang.tex,package')
%% 
%%  tracklang.dtx
%%  Copyright 2018 Nicola Talbot
%% 
%%  This work may be distributed and/or modified under the
%%  conditions of the LaTeX Project Public License, either version 1.3
%%  of this license or (at your option) any later version.
%%  The latest version of this license is in
%%    http://www.latex-project.org/lppl.txt
%%  and version 1.3 or later is part of all distributions of LaTeX
%%  version 2005/12/01 or later.
%% 
%%  This work has the LPPL maintenance status `maintained'.
%% 
%%  The Current Maintainer of this work is Nicola Talbot.
%% 
%%  This work consists of the files tracklang.dtx and tracklang.ins and the derived files tracklang.sty, tracklang.tex, tracklang-region-codes.tex, tracklang-scripts.sty, tracklang-scripts.tex.
%% 
%% \CharacterTable
%%  {Upper-case    \A\B\C\D\E\F\G\H\I\J\K\L\M\N\O\P\Q\R\S\T\U\V\W\X\Y\Z
%%   Lower-case    \a\b\c\d\e\f\g\h\i\j\k\l\m\n\o\p\q\r\s\t\u\v\w\x\y\z
%%   Digits        \0\1\2\3\4\5\6\7\8\9
%%   Exclamation   \!     Double quote  \"     Hash (number) \#
%%   Dollar        \$     Percent       \%     Ampersand     \&
%%   Acute accent  \'     Left paren    \(     Right paren   \)
%%   Asterisk      \*     Plus          \+     Comma         \,
%%   Minus         \-     Point         \.     Solidus       \/
%%   Colon         \:     Semicolon     \;     Less than     \<
%%   Equals        \=     Greater than  \>     Question mark \?
%%   Commercial at \@     Left bracket  \[     Backslash     \\
%%   Right bracket \]     Circumflex    \^     Underscore    \_
%%   Grave accent  \`     Left brace    \{     Vertical bar  \|
%%   Right brace   \}     Tilde         \~}
%% load packages that use tracklang for localisation
%% load packages that use tracklang for localisation
%% load packages that use tracklang for localisation
%% load packages that use tracklang for localisation
%% load packages that use tracklang for localisation
%% load packages that use tracklang for localisation
%% load packages that use tracklang for localisation
%% load packages that use tracklang for localisation
%% load packages that use tracklang for localisation
%% load packages that use tracklang for localisation
%% do code now to initialise
%% Pass all options to tracklang:
\ifnum\catcode`\@=11\relax
  \def\@tracklang@restore@at{}%
\else
  \expandafter\edef\csname @tracklang@restore@at\endcsname{%
    \noexpand\catcode`\noexpand\@=\number\catcode`\@\relax
  }%
 \catcode`\@=11\relax
\fi
\ifx\@tracklang@languages\undefined
\else
  \@tracklang@restore@at
  \expandafter\endinput
\fi
\expandafter\def\csname ver@tracklang.tex\endcsname{%
 2018/05/13 v1.3.6 (NLCT) Track Languages Generic Code}
\long\def\@tracklang@ifundef#1#2#3{%
  \ifcsname#1\endcsname
    \expandafter\ifx\csname #1\endcsname\relax
      #2%
    \else
      #3%
    \fi
  \else
    \expandafter\ifx\csname #1\endcsname\relax
      #2%
    \else
      #3%
    \fi
  \fi
}
\ifx\ifcsname\undefined
  \long\def\@tracklang@ifundef#1#2#3{%
    \expandafter\ifx\csname #1\endcsname\relax
      #2%
    \else
      #3%
    \fi
  }
\fi
\ifx\@@input\undefined
   \let\@tracklang@input\input
\else
   \let\@tracklang@input\@@input
\fi
\ifx\@nnil\undefined
  \def\@tracklang@nnil{\@nil}
\else
  \let\@tracklang@nnil\@nnil
\fi
\ifx\@for\undefined
  \long\def\@tracklang@for#1:=#2\do#3{%
    \expandafter\def\expandafter\@fortmp\expandafter{#2}%
    \ifx\@fortmp\empty
    \else
      \expandafter
        \@tracklang@forloop #2,\@nil,\@nil\@@ #1{#3}%
    \fi
  }
  \long\def\@tracklang@forloop#1,#2,#3\@@ #4#5{%
   \def #4{#1}%
   \ifx#4\@tracklang@nnil
   \else
     #5%
     \def #4{#2}%
     \ifx#4\@tracklang@nnil
     \else
       #5%
       \@tracklang@iforloop #3\@@ #4{#5}%
     \fi
   \fi
  }
  \long\def\@tracklang@iforloop#1,#2\@@ #3#4{%
    \def#3{#1}%
    \ifx#3\@tracklang@nnil
      \expandafter
        \@tracklang@fornoop
    \else
      #4\relax
      \expandafter\@tracklang@iforloop
    \fi
    #2\@@ #3{#4}%
  }
  \long\def\@tracklang@fornoop#1\@@ #2#3{}
\else
  \let\@tracklang@for\@for
\fi
\ifx\@namedef\undefined
  \def\@tracklang@namedef#1{\expandafter\def\csname#1\endcsname}
\else
  \let\@tracklang@namedef\@namedef
\fi
\def\@tracklang@enamedef#1{\expandafter\edef\csname#1\endcsname}
\def\@tracklang@nameuse#1{%
  \@tracklang@ifundef{#1}{}{\csname#1\endcsname}%
}
\ifx\@onelevel@sanitize\undefined
  \def\@tracklang@sanitize#1{%
    \edef#1{\expandafter\@tracklang@strip@prefix\meaning#1}%
  }
  \def\@tracklang@strip@prefix#1>{}
\else
  \let\@tracklang@sanitize\@onelevel@sanitize
\fi
\def\@tracklang@firstoftwo#1#2{#1}
\def\@tracklang@secondoftwo#1#2{#2}
\ifx\PackageError\undefined
  \def\@tracklang@err#1#2{%
    \errhelp{#2}%
    \errmessage{tracklang: #1}}
\else
  \def\@tracklang@err#1#2{\PackageError{tracklang}{#1}{#2}}
\fi
\newif\ifTrackLangShowWarnings
\TrackLangShowWarningstrue
\ifx\PackageWarning\undefined
  \def\@tracklang@pkgwarn#1#2{%
    \ifTrackLangShowWarnings
      {%
        \newlinechar=`\^^J
        \def\MessageBreak{^^J}%
        \message{^^J#1 Warning: #2 on line \the\inputlineno.^^J}%
      }%
    \fi
  }
\else
  \def\@tracklang@pkgwarn#1#2{%
    \ifTrackLangShowWarnings
      \PackageWarning{#1}{#2}%
    \fi
  }
\fi
\def\@tracklang@warn#1{\@tracklang@pkgwarn{tracklang}{#1}}%
\newif\ifTrackLangShowInfo
\TrackLangShowInfotrue
\ifx\PackageInfo\undefined
  \def\@tracklang@info#1{%
   \ifTrackLangShowInfo
     {%
       \newlinechar=`\^^J
       \def\MessageBreak{^^J}%
       \message{^^Jtracklang Info: #1 on line \the\inputlineno.^^J}%
     }%
   \fi
  }%
\else
  \def\@tracklang@info#1{%
    \ifTrackLangShowInfo
      \PackageInfo{tracklang}{#1}%
    \fi
  }%
\fi
\ifx\IfFileExists\undefined
 \long\def\@tracklang@IfFileExists#1#2#3{%
   \openin0=#1 %
   \ifeof0\relax
     \def\@tracklang@tmp{#3}%
   \else
     \closein0\relax
     \edef\@filef@und{#1 }%
     \def\@tracklang@tmp{#2}%
   \fi
   \@tracklang@tmp
 }

\else
  \let\@tracklang@IfFileExists\IfFileExists
\fi
\def\@tracklang@checklocale{%
  \ifx\TrackLangEnv\empty
  \else
    \ifx\TrackLangEnv\@tracklang@locale@posix
      \def\TrackLangEnv{}%
    \else
      \ifx\TrackLangEnv\@tracklang@locale@c
        \def\TrackLangEnv{}%
      \else
        \expandafter\@@tracklang@checklocale
           \TrackLangEnv\empty\relax
      \fi
    \fi
  \fi
}
\def\@@tracklang@checklocale#1#2\relax{%
  \ifx#1/\relax
    \def\TrackLangEnv{}%
  \fi
}
\def\@tracklang@locale@posix{POSIX}
\def\@tracklang@locale@c{C}
\ifx\directlua\undefined
  \def\@tracklang@tryshellescape#1{%
   \def\TrackLangQueryEnv{%
     \@tracklang@warn{\string\TrackLangQueryEnv\space
     non-operational as shell escape has been disabled}%
     \def\TrackLangEnv{}%
   }%
   \def\TrackLangQueryOtherEnv##1{%
     \@tracklang@warn{\string\TrackLangQueryOtherEnv{##1}\space
     non-operational as shell escape has been disabled}%
     \def\TrackLangEnv{}%
   }%
  }%
   \ifx\pdfshellescape\undefined
     \ifx\shellescape\undefined
        \def\@tracklang@tryshellescape#1{%
          \def\TrackLangQueryEnv{%
            \@tracklang@warn{\string\TrackLangQueryEnv\space
            non-operational as can't determine if the
            shell escape has been enabled. (Consider using
            eTeX or pdfTeX.)}%
            \def\TrackLangEnv{}%
          }%
          \def\TrackLangQueryOtherEnv##1{%
            \@tracklang@warn{\string\TrackLangQueryOtherEnv{##1}\space
            non-operational as can't determine if the
            shell escape has been enabled. (Consider using
            eTeX or pdfTeX.)}%
            \def\TrackLangEnv{}%
          }%
        }%
     \else
       \ifx\shellescape\relax
       \else
         \ifnum\shellescape=0\relax
         \else
           \def\@tracklang@tryshellescape#1{#1}%
         \fi
       \fi
     \fi
   \else
     \ifx\pdfshellescape\relax
       \ifx\shellescape\undefined
       \else
         \ifx\shellescape\relax
         \else
           \ifnum\shellescape=0\relax
           \else
             \def\@tracklang@tryshellescape#1{#1}%
           \fi
         \fi
       \fi
     \else
       \ifnum\pdfshellescape=0\relax
       \else
         \def\@tracklang@tryshellescape#1{#1}%
       \fi
     \fi
   \fi
   \@tracklang@tryshellescape
   {%
     \def\TrackLangQueryEnv{%
       \begingroup\endlinechar=-1\relax
       \everyeof{\noexpand}%
       \edef\x{\endgroup\def\noexpand\TrackLangEnv{%
         \@tracklang@input|"kpsewhich --var-value LC_ALL" }}\x
       \@tracklang@checklocale
       \ifx\TrackLangEnv\empty
         \begingroup\endlinechar=-1\relax
         \everyeof{\noexpand}%
         \edef\x{\endgroup\def\noexpand\TrackLangEnv{%
           \@tracklang@input|"kpsewhich --var-value LANG" }}\x
         \@tracklang@checklocale
         \ifx\TrackLangEnv\empty
           \ifx\TeXOSQueryLocale\undefined
             \@tracklang@warn{Locale environment variables
              unavailable (tried LC\string_ALL and LANG)}%
           \else
             \@tracklang@info{Using texosquery to find locale}%
             \TeXOSQueryLocale\TrackLangEnv
             \ifx\TrackLangEnv\empty
               \@tracklang@warn{Locale can't be found
               (tried querying LC\string_ALL and LANG variables and
               tried using texosquery)}%
             \fi
           \fi
         \fi
       \fi
     }%
     \def\TrackLangQueryOtherEnv#1{%
       \begingroup\endlinechar=-1\relax
       \everyeof{\noexpand}%
       \edef\x{\endgroup\def\noexpand\TrackLangEnv{%
         \@tracklang@input|"kpsewhich --var-value LC_ALL" }}\x
       \@tracklang@checklocale
       \ifx\TrackLangEnv\empty
         \begingroup\endlinechar=-1\relax
         \everyeof{\noexpand}%
         \edef\x{\endgroup\def\noexpand\TrackLangEnv{%
           \@tracklang@input|"kpsewhich --var-value #1" }}\x
         \@tracklang@checklocale
         \ifx\TrackLangEnv\empty
           \begingroup\endlinechar=-1\relax
           \everyeof{\noexpand}%
           \edef\x{\endgroup\def\noexpand\TrackLangEnv{%
             \@tracklang@input|"kpsewhich --var-value LANG"}}\x
           \@tracklang@checklocale
           \ifx\TrackLangEnv\empty
             \ifx\TeXOSQueryLocale\undefined
             \@tracklang@warn{Locale environment variables unavailable
              (tried LC\string_ALL, #1 and LANG)}%
             \else
               \@tracklang@info{Using texosquery to find locale}%
               \TeXOSQueryLocale\TrackLangEnv
               \ifx\TrackLangEnv\empty
                 \@tracklang@warn{Locale can't be found
                 (tried querying LC\string_ALL, #1 and LANG variables and
                 tried using texosquery)}%
               \fi
             \fi
           \fi
         \fi
       \fi
     }%
  }%
\else
   \def\TrackLangQueryEnv{%
     \edef\TrackLangEnv{\directlua{
       l = os.getenv("LC_ALL")
       if l == nil or l == "" or l == "C" or l == "POSIX"
                   or string.find(l, "^/") then
         l = os.getenv("LANG")
         if l == nil or l == "" or l == "C" or l == "POSIX"
                     or string.find(l, "^/") then
           l=os.setlocale(nil)
           if l == nil or l == "C" or l == "POSIX"
                       or string.find(l, "^/") then
             l = ""
           end
         end
       end
       tex.print(l)}}%
       \ifx\TrackLangEnv\empty
         \ifx\TeXOSQueryLocale\undefined
         \@tracklang@warn{Locale can't be found through Lua
          (tried querying LC\string_ALL and LANG variables and
           os.setlocale(nil))}%
         \else
           \TeXOSQueryLocale\TrackLangEnv
           \ifx\TrackLangEnv\empty
             \@tracklang@warn{Locale can't be found through Lua
             (tried querying LC\string_ALL and LANG variables and
             os.setlocale(nil) and tried using texosquery)}%
           \fi
         \fi
       \fi
   }
   \def\TrackLangQueryOtherEnv#1{%
     \edef\TrackLangEnv{\directlua{
       l = os.getenv("LC_ALL")
       if l == nil or l == "" or l == "C" or l == "POSIX"
                   or string.find(l, "^/") then
         l = os.getenv("#1")
         if l == nil or l == "" or l == "C" or l == "POSIX"
                     or string.find(l, "^/") then
           l = os.getenv("LANG")
           if l == nil or l == "" or l == "C" or l == "POSIX"
                       or string.find(l, "^/") then
             l=os.setlocale(nil)
             if l == nil or l == "C" or l == "POSIX"
                         or string.find(l, "^/") then
               l = ""
             end
           end
         end
       end
       tex.print(l}}%
       \ifx\TrackLangEnv\empty
         \ifx\TeXOSQueryLocale\undefined
         \@tracklang@warn{Locale can't be found through Lua
          (tried querying LC\string_ALL, #1 and LANG variables and
           os.setlocale(nil))}%
         \else
           \TeXOSQueryLocale\TrackLangEnv
           \ifx\TrackLangEnv\empty
             \@tracklang@warn{Locale can't be found through Lua
             (tried querying LC\string_ALL, #1 and LANG variables and
             os.setlocale(nil) and tried using texosquery)}%
           \fi
         \fi
       \fi
   }
\fi
\def\TrackLangParseFromEnv{%
  \ifx\TrackLangEnv\undefined
     \@tracklang@warn{\string\TrackLangParseFromEnv\space
     non-operational as \string\TrackLangEnv\space hasn't been
     defined}%
     \def\TrackLangEnvLang{}%
     \def\TrackLangEnvTerritory{}%
     \def\TrackLangEnvCodeSet{}%
     \def\TrackLangEnvModifier{}%
  \else
    \ifx\TrackLangEnv\empty
      \@tracklang@warn{\string\TrackLangParseFromEnv\space
      non-operational as \string\TrackLangEnv\space is empty}%
      \def\TrackLangEnvLang{}%
      \def\TrackLangEnvTerritory{}%
      \def\TrackLangEnvCodeSet{}%
      \def\TrackLangEnvModifier{}%
    \else
      \@tracklang@parse@locale{\TrackLangEnv}%
      \let\TrackLangEnvLang\@TrackLangEnvLang
      \let\TrackLangEnvTerritory\@TrackLangEnvTerritory
      \let\TrackLangEnvCodeSet\@TrackLangEnvCodeSet
      \let\TrackLangEnvModifier\@TrackLangEnvModifier
    \fi
  \fi
}
\def\@tracklang@parse@locale#1{%
  \def\@TrackLangEnvLang{}%
  \def\@TrackLangEnvSubLang{}%
  \def\@TrackLangEnvFirstSubLang{}%
  \def\@TrackLangEnvTerritory{}%
  \def\@TrackLangEnvCodeSet{}%
  \def\@TrackLangEnvVariant{}%
  \def\@TrackLangEnvModifier{}%
  \def\@TrackLangEnvScript{}%
  \def\@TrackLangEnvAdditional{}%
  \expandafter\ifx\expandafter\relax#1\relax
  \else
    \expandafter\@tracklang@parseenv
      #1..\relax\@tracklang@end@parseenv\@tracklang@result
    \ifx\@tracklang@result\empty
    \else
      \expandafter\@tracklang@split@underscoreorhyp\expandafter
       {\@tracklang@result}%
      \let\@TrackLangEnvLang\@tracklang@split@pre
      \let\@TrackLangEnvTerritory\@tracklang@split@post
    \fi
  \fi
}
\def\@tracklang@split@underscoreorhyp#1{%
  \@tracklang@split@underscore{#1}%
  \ifx\@tracklang@split@post\empty
    \@tracklang@split@hyphen{#1}%
    \ifx\@tracklang@split@post\empty
      \@tracklang@split@otherunderscore{#1}%
    \fi
  \fi
}
{
  \catcode`\_8\relax
  \gdef\@tracklang@split@underscore#1{%
    \@@tracklang@split@underscore#1__\relax\@tracklang@end@split@underscore
  }
  \gdef\@@tracklang@split@underscore#1_#2_#3\@tracklang@end@split@underscore{%
    \def\@tracklang@split@pre{#1}%
    \ifx\relax#3\relax
      \def\@tracklang@split@post{#2}%
    \else
      \@tracklang@split@underscore@remainder#2_#3%
    \fi
  }
  \gdef\@tracklang@split@underscore@remainder#1__\relax{%
    \def\@tracklang@split@post{#1}%
  }
}
{
  \catcode`\_12\relax
  \gdef\@tracklang@split@otherunderscore#1{%
    \@@tracklang@split@otherunderscore#1__\relax\@tracklang@end@split@underscore
  }
  \gdef\@@tracklang@split@otherunderscore#1_#2_#3\@tracklang@end@split@underscore{%
    \def\@tracklang@split@pre{#1}%
    \ifx\relax#3\relax
      \def\@tracklang@split@post{#2}%
    \else
      \@tracklang@split@otherunderscore@remainder#2_#3%
    \fi
  }
  \gdef\@tracklang@split@otherunderscore@remainder#1__\relax{%
    \def\@tracklang@split@post{#1}%
  }
}
{
  \catcode`\-12\relax
  \gdef\@tracklang@split@hyphen#1{%
    \@@tracklang@split@hyphen#1--\relax\@tracklang@end@split@hyphen
  }
  \gdef\@@tracklang@split@hyphen#1-#2-#3\@tracklang@end@split@hyphen{%
    \def\@tracklang@split@pre{#1}%
    \ifx\relax#3\relax
      \def\@tracklang@split@post{#2}%
    \else
      \@tracklang@split@hyphen@remainder#2-#3%
    \fi
  }
  \gdef\@tracklang@split@hyphen@remainder#1--\relax{%
    \def\@tracklang@split@post{#1}%
  }
}
\gdef\@tracklang@parseenv#1.#2.#3\@tracklang@end@parseenv#4{%
  \def\@TrackLangEnvCodeSet{#2}%
  \def#4{#1}%
  \ifx\@TrackLangEnvCodeSet\empty
    \tracklangparsemod#4%
  \else
    \tracklangparsemod\@TrackLangEnvCodeSet
  \fi
}
{\catcode`\@=12\relax
  \gdef\tracklangparsemod#1{
    \expandafter\tracklangparseenvatmod#1@@\relax\tracklangendparseenvatmod
    \let#1\tracklangtmp
  }%
  \gdef\tracklangparseenvatmod#1@#2@#3\tracklangendparseenvatmod{%
    \def\tracklangtmp{#1}%
    \expandafter\def\csname @TrackLangEnvModifier\endcsname{#2}%
    \csname @tracklang@sanitize\expandafter\endcsname
      \csname @TrackLangEnvModifier\endcsname
  }
}
\def\@tracklang@languages{}
\def\@tracklang@dialects{}
\def\@tracklang@ifinlist#1#2#3#4{%
  \def\@tracklang@doifinlist##1,#1,##2\end@tracklang@doifinlist{%
     \def\@before{##1}%
     \def\@after{##2}%
  }%
  \expandafter\@tracklang@doifinlist\expandafter,#2,#1,\@nil
    \end@tracklang@doifinlist
  \ifx\@after\@tracklang@nnil
    #4%
  \else
    #3%
  \fi
}
\def\@tracklang@add#1#2{%
  \edef\@tracklang@element{#1}%
  \ifx\@tracklang@element\empty
  \else
    \expandafter\@tracklang@ifinlist\expandafter{\@tracklang@element}#2%
    {%
    }%
    {%
     \ifx\empty#2\relax
       \let#2\@tracklang@element
     \else
       \edef#2{#2,\@tracklang@element}%
     \fi
    }%
  \fi
}
\def\AddTrackedDialect#1#2{%
 \@tracklang@add{#1}{\@tracklang@dialects}%
 \@tracklang@add{#2}{\@tracklang@languages}%
 \@tracklang@enamedef{@tracklang@fromdialect@#1}{#2}%
 \@tracklang@ifundef{@tracklang@todialect@#2}%
 {\@tracklang@enamedef{@tracklang@todialect@#2}{#1}}%
 {%
   \def\@tracklang@lang{#1}%
   \expandafter\@tracklang@add\expandafter\@tracklang@lang
     \csname @tracklang@todialect@#2\endcsname
 }%
 \edef\TrackLangLastTrackedDialect{#1}%
}
\def\AddTrackedLanguage#1{%
  \AddTrackedDialect{#1}{#1}%
}
\def\@tracklang@known@langs{}
\def\TrackLangNewLanguage#1#2#3#4#5#6#7{%
 \@tracklang@add{#1}{\@tracklang@known@langs}%
 \edef\@tracklang@tmp{#2}%
 \ifx\@tracklang@tmp\empty
 \else
   \@tracklang@enamedef{@tracklang@knownisolang@#2}{#1}%
   \@tracklang@enamedef{@tracklang@knowniso@639@1@#1}{#2}%
 \fi
 \edef\@tracklang@tmp{#3}%
 \ifx\@tracklang@tmp\empty
 \else
   \@tracklang@enamedef{@tracklang@knownisolang@#3}{#1}%
   \@tracklang@enamedef{@tracklang@knowniso@639@2@#1}{#3}%
 \fi
 \edef\@tracklang@tmp{#4}%
 \ifx\@tracklang@tmp\empty
 \else
   \@tracklang@enamedef{@tracklang@knowniso@639@2B@#1}{#4}%
 \fi
 \edef\@tracklang@tmp{#5}%
 \ifx\@tracklang@tmp\empty
 \else
   \@tracklang@enamedef{@tracklang@knownisolang@#5}{#1}%
   \@tracklang@enamedef{@tracklang@knowniso@639@3@#1}{#5}%
 \fi
 \edef\@tracklang@tmp{#6}%
 \ifx\@tracklang@tmp\empty
 \else
   \@tracklang@enamedef{@tracklang@knowniso@3166@#1}{#6}%
 \fi
 \edef\@tracklang@tmp{#7}%
 \ifx\@tracklang@tmp\empty
 \else
   \@tracklang@enamedef{@tracklang@knowniso@script@#1}{#7}%
 \fi
}
\def\TrackLangIfKnownLang#1#2#3{%
  \expandafter\@tracklang@ifinlist\expandafter{#1}{\@tracklang@known@langs}%
  {#2}%
  {#3}%
}
\def\TrackLangIfKnownIsoTwoLetterLang#1#2#3{%
  \@tracklang@ifundef{@tracklang@knowniso@639@1@#1}%
  {#3}%
  {#2}%
}
\def\TrackLangGetKnownIsoTwoLetterLang#1{%
  \@tracklang@nameuse{@tracklang@knowniso@639@1@#1}%
}
\def\TrackLangIfKnownIsoThreeLetterLang#1#2#3{%
  \@tracklang@ifundef{@tracklang@knowniso@639@2@#1}%
  {#3}%
  {#2}%
}
\def\TrackLangGetKnownIsoThreeLetterLang#1{%
  \@tracklang@nameuse{@tracklang@knowniso@639@2@#1}%
}
\def\TrackLangIfKnownIsoThreeLetterLangB#1#2#3{%
  \@tracklang@ifundef{@tracklang@knowniso@639@2B@#1}%
  {#3}%
  {#2}%
}
\def\TrackLangGetKnownIsoThreeLetterLangB#1{%
  \@tracklang@nameuse{@tracklang@knowniso@639@2B@#1}%
}
\def\TrackLangIfKnownLangFromIso#1#2#3{%
  \@tracklang@ifundef{@tracklang@knownisolang@#1}%
  {#3}%
  {#2}%
}
\def\TrackLangGetKnownLangFromIso#1{%
  \@tracklang@nameuse{@tracklang@knownisolang@#1}%
}
\def\TrackLangIfHasKnownCountry#1#2#3{%
  \@tracklang@ifundef{@tracklang@knowniso@3166@#1}%
  {#3}%
  {#2}%
}
\def\TrackLangGetKnownCountry#1{%
  \@tracklang@nameuse{@tracklang@knowniso@3166@#1}%
}
\def\TrackLangGetDefaultScript#1{%
  \@tracklang@nameuse{@tracklang@knowniso@script@#1}%
}
\def\TrackLangIfHasDefaultScript#1#2#3{%
  \@tracklang@ifundef{@tracklang@knowniso@script@#1}{#3}{#2}%
}
\def\AddTrackedIsoLanguage#1#2#3{%
  \@tracklang@enamedef{@tracklang@#1@isofromlang@#3}{#2}%
  \@tracklang@ifundef{@tracklang@#1@isotolang@#2}%
  {\@tracklang@enamedef{@tracklang@#1@isotolang@#2}{#3}}%
  {%
    \def\@tracklang@lang{#3}%
    \expandafter\@tracklang@add\expandafter\@tracklang@lang
      \csname @tracklang@#1@isotolang@#2\endcsname
  }%
}
\def\TrackedLanguageFromIsoCode#1#2{%
  \@tracklang@nameuse{@tracklang@#1@isotolang@#2}%
}
\def\TrackedIsoCodeFromLanguage#1#2{%
  \@tracklang@nameuse{@tracklang@#1@isofromlang@#2}%
}
\def\TrackedLanguageFromDialect#1{%
 \@tracklang@nameuse{@tracklang@fromdialect@#1}%
}
\def\TrackedDialectsFromLanguage#1{%
 \@tracklang@nameuse{@tracklang@todialect@#1}%
}
\def\TwoLetterIsoCountryCode{3166-1}
\def\TwoLetterIsoLanguageCode{639-1}
\def\ThreeLetterIsoLanguageCode{639-2}
\def\ThreeLetterExtIsoLanguageCode{639-3}
\def\SetTrackedDialectModifier#1#2{%
  \@tracklang@enamedef{@tracklang@modifier@#1}{#2}%
}
\def\GetTrackedDialectModifier#1{%
  \@tracklang@nameuse{@tracklang@modifier@#1}%
}
\def\IfHasTrackedDialectModifier#1#2#3{%
  \@tracklang@ifundef{@tracklang@modifier@#1}{#3}{#2}%
}
\def\SetTrackedDialectScript#1#2{%
  \@tracklang@enamedef{@tracklang@script@#1}{#2}%
}
\def\GetTrackedDialectScript#1{%
  \@tracklang@nameuse{@tracklang@script@#1}%
}
\def\IfHasTrackedDialectScript#1#2#3{%
  \@tracklang@ifundef{@tracklang@script@#1}{#3}{#2}%
}
\def\IfTrackedDialectIsScriptCs#1#2#3#4{%
  \IfHasTrackedDialectScript{#1}%
  {%
    \expandafter\ifx\expandafter#2\csname @tracklang@script@#1\endcsname
      #3%
    \else
      #4%
    \fi
  }%
  {%
    \TrackLangIfHasDefaultScript{\TrackedLanguageFromDialect{#1}}%
    {%
      \expandafter\ifx\expandafter
        #2\csname @tracklang@knowniso@script@\TrackedLanguageFromDialect{#1}\endcsname
         #3%
      \else
         #4%
      \fi
    }%
    {#4}%
  }%
}
\def\SetTrackedDialectVariant#1#2{%
  \@tracklang@enamedef{@tracklang@variant@#1}{#2}%
}
\def\GetTrackedDialectVariant#1{%
  \@tracklang@nameuse{@tracklang@variant@#1}%
}
\def\IfHasTrackedDialectVariant#1#2#3{%
  \@tracklang@ifundef{@tracklang@variant@#1}{#3}{#2}%
}
\def\SetTrackedDialectSubLang#1#2{%
  \@tracklang@enamedef{@tracklang@sublang@#1}{#2}%
}
\def\GetTrackedDialectSubLang#1{%
  \@tracklang@nameuse{@tracklang@sublang@#1}%
}
\def\IfHasTrackedDialectSubLang#1#2#3{%
  \@tracklang@ifundef{@tracklang@sublang@#1}{#3}{#2}%
}
\def\SetTrackedDialectAdditional#1#2{%
  \@tracklang@enamedef{@tracklang@extra@#1}{#2}%
}
\def\GetTrackedDialectAdditional#1{%
  \@tracklang@nameuse{@tracklang@extra@#1}%
}
\def\IfHasTrackedDialectAdditional#1#2#3{%
  \@tracklang@ifundef{@tracklang@extra@#1}{#3}{#2}%
}
\def\GetTrackedLanguageTag#1{%
  \IfTrackedLanguageHasIsoCode{639-1}{\TrackedLanguageFromDialect{#1}}%
  {\TrackedIsoCodeFromLanguage{639-1}{\TrackedLanguageFromDialect{#1}}}%
  {%
    \IfTrackedLanguageHasIsoCode{639-2}{\TrackedLanguageFromDialect{#1}}%
    {\TrackedIsoCodeFromLanguage{639-2}{\TrackedLanguageFromDialect{#1}}}%
    {%
      \IfTrackedLanguageHasIsoCode{639-3}{\TrackedLanguageFromDialect{#1}}%
      {\TrackedIsoCodeFromLanguage{639-3}{\TrackedLanguageFromDialect{#1}}}%
      {und}% undefined
    }%
  }%
  \@tracklang@ifundef{@tracklang@sublang@#1}%
  {}%
  {-\csname @tracklang@sublang@#1\endcsname}%
  \@tracklang@ifundef{@tracklang@script@#1}%
  {}%
  {-\csname @tracklang@script@#1\endcsname}%
  \IfTrackedLanguageHasIsoCode{3166-1}{#1}%
  {-\TrackedIsoCodeFromLanguage{3166-1}{#1}}%
  {}%
  \@tracklang@ifundef{@tracklang@variant@#1}%
  {}%
  {-\csname @tracklang@variant@#1\endcsname}%
  \@tracklang@ifundef{@tracklang@extra@#1}%
  {}%
  {-\csname @tracklang@extra@#1\endcsname}%
}
\def\SetCurrentTrackedDialect#1{%
  \edef\CurrentTrackedDialect{#1}%
  \IfTrackedDialect{\CurrentTrackedDialect}%
  {}%
  {%
    \IfHookHasMappingFromTrackedDialect{\CurrentTrackedDialect}%
    {%
      \IfTrackedDialect{\GetTrackedDialectFromMapping\CurrentTrackedDialect}%
      {%
        \edef\CurrentTrackedDialect{\GetTrackedDialectFromMapping
          {\CurrentTrackedDialect}}%
      }%
      {%
        \IfTrackedLanguage{#1}%
        {%
          \edef\@tracklang@dialects{\TrackedDialectsFromLanguage{#1}}%
          \@tracklang@for\@tracklang@dialect:=\@tracklang@dialects\do{%
            \let\CurrentTrackedDialect\@tracklang@dialect
          }%
        }%
        {}%
      }%
    }%
    {%
      \IfTrackedLanguage{#1}%
      {%
        \edef\@tracklang@dialects{\TrackedDialectsFromLanguage{#1}}%
        \@tracklang@for\@tracklang@dialect:=\@tracklang@dialects\do{%
          \let\CurrentTrackedDialect\@tracklang@dialect
        }%
      }%
      {}%
    }%
  }%
  \IfTrackedDialect{\CurrentTrackedDialect}%
  {%
    \edef\CurrentTrackedLanguage{%
      \TrackedLanguageFromDialect{\CurrentTrackedDialect}}%
    \edef\CurrentTrackedDialectModifier{%
      \GetTrackedDialectModifier{\CurrentTrackedDialect}}%
    \edef\CurrentTrackedDialectVariant{%
      \GetTrackedDialectVariant{\CurrentTrackedDialect}}%
    \IfHasTrackedDialectScript{\CurrentTrackedDialect}%
    {%
      \edef\CurrentTrackedDialectScript{%
        \GetTrackedDialectScript{\CurrentTrackedDialect}}%
    }%
    {%
      \edef\CurrentTrackedDialectScript{%
        \TrackLangGetDefaultScript\CurrentTrackedLanguage}%
    }%
    \edef\CurrentTrackedDialectSubLang{%
      \GetTrackedDialectSubLang{\CurrentTrackedDialect}}%
    \edef\CurrentTrackedDialectAdditional{%
      \GetTrackedDialectAdditional{\CurrentTrackedDialect}}%
    \edef\CurrentTrackedLanguageTag{%
      \GetTrackedLanguageTag{\CurrentTrackedDialect}}%
    \IfTrackedLanguageHasIsoCode{3166-1}{\CurrentTrackedDialect}%
    {%
      \edef\CurrentTrackedRegion{%
       \TrackedIsoCodeFromLanguage{3166-1}{\CurrentTrackedDialect}}%
    }%
    {\def\CurrentTrackedRegion{}}%
    \IfTrackedLanguageHasIsoCode{639-1}{\CurrentTrackedLanguage}%
    {%
      \edef\CurrentTrackedIsoCode{%
       \TrackedIsoCodeFromLanguage{639-1}{\CurrentTrackedLanguage}}%
    }%
    {%
      \IfTrackedLanguageHasIsoCode{639-2}{\CurrentTrackedLanguage}%
      {%
        \edef\CurrentTrackedIsoCode{%
         \TrackedIsoCodeFromLanguage{639-2}{\CurrentTrackedLanguage}}%
      }%
      {%
        \IfTrackedLanguageHasIsoCode{639-3}{\CurrentTrackedLanguage}%
        {%
          \edef\CurrentTrackedIsoCode{%
           \TrackedIsoCodeFromLanguage{639-3}{\CurrentTrackedLanguage}}%
        }%
        {%
          \def\CurrentTrackedIsoCode{}%
        }%
      }%
    }%
  }%
  {%
    \@tracklang@warn{Unknown dialect label `#1' passed to
      \string\SetCurrentTrackedDialect}%
    \edef\CurrentTrackedLanguage{\languagename}%
    \def\CurrentTrackedDialectModifier{}%
    \def\CurrentTrackedDialectVariant{}%
    \def\CurrentTrackedDialectScript{}%
    \def\CurrentTrackedDialectSubLang{}%
    \def\CurrentTrackedDialectAdditional{}%
    \def\CurrentTrackedIsoCode{}%
    \def\CurrentTrackedRegion{}%
    \def\CurrentTrackedLanguageTag{und}%
  }%
}
\def\AddTrackedLanguageIsoCodes#1{%
  \@tracklang@ifundef{@tracklang@knowniso@639@1@#1}%
  {}%
  {%
    \AddTrackedIsoLanguage\TwoLetterIsoLanguageCode
      {\csname @tracklang@knowniso@639@1@#1\endcsname}{#1}%
  }%
  \@tracklang@ifundef{@tracklang@knowniso@639@2@#1}%
  {}%
  {%
    \AddTrackedIsoLanguage\ThreeLetterIsoLanguageCode
       {\csname @tracklang@knowniso@639@2@#1\endcsname}{#1}%
    \@tracklang@ifundef{@tracklang@knowniso@639@2B@#1}%
    {}%
    {%
      \AddTrackedIsoLanguage{\ThreeLetterIsoLanguageCode-T}%
         {\csname @tracklang@knowniso@639@2@#1\endcsname}{#1}%
      \AddTrackedIsoLanguage{\ThreeLetterIsoLanguageCode-B}%
         {\csname @tracklang@knowniso@639@2B@#1\endcsname}{#1}%
    }%
  }%
  \@tracklang@ifundef{@tracklang@knowniso@639@3@#1}%
  {}%
  {%
    \AddTrackedIsoLanguage\ThreeLetterExtIsoLanguageCode
      {\csname @tracklang@knowniso@639@3@#1\endcsname}{#1}%
  }%
}
\def\AddTrackedCountryIsoCode#1{%
  \@tracklang@ifundef{@tracklang@knowniso@3166@#1}%
  {}%
  {%
    \AddTrackedIsoLanguage{3166-1}%
      {\csname @tracklang@knowniso@3166@#1\endcsname}{#1}%
  }%
}
\def\TrackPredefinedDialect#1{%
  \@tracklang@ifundef{@tracklang@add@#1}%
  {%
    \@tracklang@err{Dialect or language `#1' is not predefined}{}%
  }%
  {\@tracklang@nameuse{@tracklang@add@#1}}%
}
\def\@tracklang@hassecondchar#1#2\@end@tracklang@hassecondchar#3#4{%
  \ifx\relax#2\relax
    #4%
  \else
    #3%
  \fi
}
\def\@tracklang@hasthirdchar#1#2#3\@end@tracklang@hasthirdchar#4#5{%
  \ifx\relax#3\relax
    #5%
  \else
    #4%
  \fi
}
\def\@tracklang@hasfourthchar#1#2#3#4\@end@tracklang@hasfourthchar#5#6{%
  \ifx\relax#4\relax
    #6%
  \else
    #5%
  \fi
}
\def\@tracklang@hasfifthchar#1#2#3#4#5\@end@tracklang@hasfifthchar#6#7{%
  \ifx\relax#5\relax
    #7%
  \else
    #6%
  \fi
}
\def\@tracklang@hasninthchar#1#2#3#4#5#6#7#8#9\@end@tracklang@hasninthchar{%
  \ifx\relax#9\relax
    \expandafter\@tracklang@secondoftwo
  \else
    \expandafter\@tracklang@firstoftwo
  \fi
}
\def\@tracklang@ifalpha#1#2#3{%
  \ifx\relax#1\relax
    #3%
  \else
   \ifnum\lccode`#1<`a\relax
     #3%
   \else
     \ifnum\lccode`#1>`z\relax
      #3%
     \else
       #2%
     \fi
   \fi
  \fi
}
\def\@tracklang@ifdigit#1#2#3{%
  \ifx\relax#1\relax
    #3%
  \else
   \ifnum`#1<`0\relax
     #3%
   \else
     \ifnum`#1>`9\relax
      #3%
     \else
       #2%
     \fi
   \fi
  \fi
}
\def\@tracklang@ifalldigits#1{%
 \expandafter\ifx\relax#1\relax
   \expandafter\@tracklang@secondoftwo
 \else
   \expandafter\@@tracklang@ifalldigits#1\@tracklang@nnil
 \fi
}
\def\@@tracklang@ifalldigits#1{%
  \ifx#1\@tracklang@nnil
   \def\@tracklang@next{\expandafter\@tracklang@firstoftwo}%
  \else
    \@tracklang@ifdigit{#1}%
    {%
      \let\@tracklang@next\@@tracklang@ifalldigits
    }%
    {%
      \def\@tracklang@next##1\@tracklang@nnil{%
        \expandafter\@tracklang@secondoftwo}%
    }%
  \fi
  \@tracklang@next
}
\def\@tracklang@ifalphanumeric#1#2#3{%
  \@tracklang@ifalpha{#1}%
  {#2}%
  {%
    \@tracklang@ifdigit{#1}{#2}{#3}%
  }%
}
\def\TrackLangIfAlphaNumericChar#1#2#3{%
  \expandafter\ifx\expandafter\relax#1\relax
    #3%
  \else
    \expandafter\@tracklang@hassecondchar#1\relax\relax
      \@end@tracklang@hassecondchar
    {#3}%
    {\expandafter\@tracklang@ifalphanumeric#1{#2}{#3}}%
  \fi
}
\def\TrackLangIfLanguageTag#1#2#3{%
  \expandafter\@tracklang@hasthirdchar#1\relax\relax\relax
    \@end@tracklang@hasthirdchar
  {%
    \expandafter\@tracklang@hasfourthchar#1\relax\@end@tracklang@hasfourthchar
    {#3}%
    {%
     \expandafter\@tracklang@iflanguage@iii@tag#1{#2}{#3}%
    }%
  }%
  {%
    \expandafter\@tracklang@hassecondchar#1\relax\relax
      \@end@tracklang@hassecondchar
    {%
     \expandafter\@tracklang@iflanguage@ii@tag#1{#2}{#3}%
    }%
    {#3}%
  }%
}
\def\@tracklang@iflanguage@ii@tag#1#2#3#4{%
  \ifnum\lccode`#1=`#1\relax
    \ifnum\lccode`#2=`#2\relax
      #3%
    \else
      #4%
    \fi
  \else
    #4%
  \fi
}
\def\@tracklang@iflanguage@iii@tag#1#2#3#4#5{%
  \ifnum\lccode`#1=`#1\relax
    \ifnum\lccode`#2=`#2\relax
      \ifnum\lccode`#3=`#3\relax
        #4%
      \else
        #5%
      \fi
    \else
      #5%
    \fi
  \else
    #5%
  \fi
}
\def\TrackLangIfRegionTag#1#2#3{%
  \expandafter\@tracklang@hasthirdchar#1\relax\relax\relax
    \@end@tracklang@hasthirdchar
  {%
    \expandafter\@tracklang@hasfourthchar#1\relax\@end@tracklang@hasfourthchar
    {%
      #3%
    }%
    {%
      \@tracklang@ifalldigits{#1}{#2}{#3}%
    }%
  }%
  {%
    \expandafter\@tracklang@hassecondchar#1\relax\relax
      \@end@tracklang@hassecondchar
    {%
     \expandafter\@tracklang@ifregion@ii@tag#1{#2}{#3}%
    }%
    {#3}%
  }%
}
\def\@tracklang@ifregion@ii@tag#1#2#3#4{%
  \ifnum\uccode`#1=`#1\relax
    \ifnum\uccode`#2=`#2\relax
      #3%
    \else
      #4%
    \fi
  \else
    #4%
  \fi
}
\def\@tracklang@ifregion@iii@tag#1#2#3#4#5{%
  \ifnum\uccode`#1=`#1\relax
    \ifnum\uccode`#2=`#2\relax
      \ifnum\uccode`#3=`#3\relax
        #4%
      \else
        #5%
      \fi
    \else
      #5%
    \fi
  \else
    #5%
  \fi
}
\def\TrackLangIfScriptTag#1#2#3{%
  \expandafter\@tracklang@hasfifthchar#1\relax\relax\relax\relax\relax
    \@end@tracklang@hasfifthchar
  {#3}%
  {%
    \expandafter\@tracklang@hasfourthchar#1\relax\relax\relax\relax
      \@end@tracklang@hasfourthchar
    {%
     \expandafter\@tracklang@ifscripttag#1{#2}{#3}%
    }%
    {#3}%
  }%
}
\def\@tracklang@ifscripttag#1#2#3#4#5#6{%
  \ifnum\uccode`#1=`#1\relax
    \ifnum\lccode`#2=`#2\relax
      \ifnum\lccode`#3=`#3\relax
        \ifnum\lccode`#4=`#4\relax
          #5%
        \else
          #6%
        \fi
      \else
        #6%
      \fi
    \else
      #6%
    \fi
  \else
    #6%
  \fi
}
\def\TrackLangIfVariantTag#1#2#3{%
  \expandafter\@tracklang@hasfifthchar#1\relax\relax\relax\relax\relax
    \@end@tracklang@hasfifthchar
  {%
    \expandafter\@tracklang@hasninthchar#1\relax\relax\relax\relax\relax
      \relax\relax\relax\relax
      \@end@tracklang@hasninthchar
    {#3}%
    {#2}%
  }%
  {%
    \expandafter\@tracklang@hasfourthchar#1\relax\relax\relax\relax
      \@end@tracklang@hasfourthchar
    {%
      \expandafter\@tracklang@ifvariant@iv@tag#1{#2}{#3}%
    }%
    {#3}%
  }%
}
\def\@tracklang@ifvariant@iv@tag#1#2#3#4#5#6{%
  \@tracklang@ifdigit{#1}%
  {#5}
  {#6}%
}
\def\@tracklang@parse@extlang{%
   \TrackLangIfLanguageTag{\@tracklang@split@pre}
   {%
     \ifx\@TrackLangEnvSubLang\empty
       \let\@TrackLangEnvSubLang\@tracklang@split@pre
       \let\@TrackLangEnvFirstSubLang\@TrackLangEnvSubLang
     \else
       \edef\@TrackLangEnvSubLang{\@TrackLangEnvSubLang-\@tracklang@split@pre}%
     \fi
     \ifx\@tracklang@split@post\empty
     \else
       \expandafter\@tracklang@split@underscoreorhyp\expandafter
         {\@tracklang@split@post}%
       \ifx\@tracklang@split@pre\empty
       \else
         \@tracklang@parse@extlang
       \fi
     \fi
   }%
   {}%
}
\def\@tracklang@parse@variant{%
   \TrackLangIfVariantTag{\@tracklang@split@pre}
   {%
     \ifx\@TrackLangEnvVariant\empty
       \let\@TrackLangEnvVariant\@tracklang@split@pre
     \else
       \edef\@TrackLangEnvVariant{\@TrackLangEnvVariant
         -\@tracklang@split@pre}%
     \fi
     \ifx\@tracklang@split@post\empty
     \else
       \expandafter\@tracklang@split@underscoreorhyp\expandafter
         {\@tracklang@split@post}%
       \ifx\@tracklang@split@pre\empty
       \else
         \@tracklang@parse@variant
       \fi
     \fi
   }%
   {}%
}
\def\TrackLanguageTag#1{%
  \edef\@tracklang@tag{#1}%
  \ifx\@tracklang@tag\empty
    \@tracklang@warn{Empty tag in \string\TrackLanguageTag}%
  \else
    \expandafter\@TrackLanguageTag\expandafter{\@tracklang@tag}%
  \fi
}
\def\@TrackLanguageTag#1{%
  \@tracklang@ifundef{@tracklang@add@#1}%
  {%
     \@tracklang@parselangtag{#1}%
     \@tracklang@track@locale
  }%
  {%
    \@tracklang@nameuse{@tracklang@add@#1}%
  }%
}
\def\@tracklang@parselangtag#1{%
  \def\@TrackLangEnvLang{}%
  \def\@TrackLangEnvSubLang{}%
  \def\@TrackLangEnvFirstSubLang{}%
  \def\@TrackLangEnvTerritory{}%
  \def\@TrackLangEnvCodeSet{}%
  \def\@TrackLangEnvVariant{}%
  \def\@TrackLangEnvModifier{}%
  \def\@TrackLangEnvScript{}%
  \def\@TrackLangEnvAdditional{}%
  \@tracklang@split@underscoreorhyp{#1}%
  \let\@TrackLangEnvLang\@tracklang@split@pre
  \ifx\@tracklang@split@post\empty
  \else
     \expandafter\@tracklang@split@underscoreorhyp\expandafter
       {\@tracklang@split@post}%
     \@tracklang@parse@extlang
     \TrackLangIfScriptTag{\@tracklang@split@pre}%
     {%
       \let\@TrackLangEnvScript\@tracklang@split@pre
       \ifx\@tracklang@split@post\empty
       \else
         \expandafter\@tracklang@split@underscoreorhyp\expandafter
           {\@tracklang@split@post}%
       \fi
     }%
     {}%
     \TrackLangIfRegionTag{\@tracklang@split@pre}%
     {%
       \expandafter\@tracklang@hasthirdchar\@tracklang@split@pre
          \relax\relax\relax
          \@end@tracklang@hasthirdchar
       {%
         \ifx\TrackLangIfKnownNumericRegion\undefined
           \@tracklang@input tracklang-region-codes.tex
         \fi
         \TrackLangIfKnownNumericRegion{\@tracklang@split@pre}%
         {%
           \edef\@TrackLangEnvTerritory{%
             \TrackLangNumericToAlphaIIRegion{\@tracklang@split@pre}%
           }%
         }%
         {%
           \let\@TrackLangEnvTerritory\@tracklang@split@pre
           \@tracklang@warn{Unrecognised numeric region code
             `\@tracklang@split@pre'}%
         }%
       }%
       {%
         \let\@TrackLangEnvTerritory\@tracklang@split@pre
       }%
     \expandafter\@tracklang@split@underscoreorhyp\expandafter
         {\@tracklang@split@post}%
     }%
     {}%
     \@tracklang@parse@variant
     \let\@TrackLangEnvAdditional\@tracklang@split@post
  \fi
}%
\def\GetTrackedDialectFromLanguageTag#1#2{%
  \def#2{}%
  \def\TrackedDialectClosestSubMatch{}%
  \@tracklang@parselangtag{#1}%
  \edef\@tracklang@dialect{%
   \@TrackLangEnvLang
   \@TrackLangEnvSubLang
   \@TrackLangEnvScript
   \@TrackLangEnvTerritory
   \@TrackLangEnvModifier
   \@TrackLangEnvVariant}%
  \IfTrackedDialect{\@tracklang@dialect}%
  {%
      \let#2\@tracklang@dialect
  }%
  {%
      \edef\@tracklang@lang{\TrackLangGetKnownLangFromIso\@TrackLangEnvLang}%
      \edef\@tracklang@defscript{\TrackLangGetDefaultScript\@tracklang@lang}%
     \def\@tracklang@bestmatch{0}%
      \edef\@tracklang@dialects{\TrackedDialectsFromLanguage\@tracklang@lang}%
      \@tracklang@for\@tracklang@dialect:=\@tracklang@dialects\do{%
        \def\@tracklang@currentmatch{0}%
        \edef\@tracklang@tmp{%
          \GetTrackedDialectScript{\@tracklang@dialect}}%
        \ifx\@tracklang@tmp\@TrackLangEnvScript
          \def\@tracklang@currentmatch{1}%
        \else
          \ifx\@TrackLangEnvScript\empty
            \ifx\@tracklang@tmp\@tracklang@defscript
              \def\@tracklang@currentmatch{1}%
            \fi
          \fi
        \fi
        \edef\@tracklang@tmp{%
          \GetTrackedDialectSubLang{\@tracklang@dialect}}%
        \ifx\@tracklang@tmp\@TrackLangEnvSubLang
          \edef\@tracklang@currentmatch{\@tracklang@currentmatch 1}%
        \else
          \edef\@tracklang@currentmatch{\@tracklang@currentmatch 0}%
        \fi
        \edef\@tracklang@tmp{%
          \GetTrackedDialectVariant{\@tracklang@dialect}}%
        \ifx\@tracklang@tmp\@TrackLangEnvVariant
          \edef\@tracklang@currentmatch{\@tracklang@currentmatch 1}%
        \else
          \edef\@tracklang@currentmatch{\@tracklang@currentmatch 0}%
        \fi
        \edef\@tracklang@tmp{%
          \TrackedIsoCodeFromLanguage{3166-1}{\@tracklang@dialect}}%
        \ifx\@tracklang@tmp\@TrackLangEnvTerritory
          \edef\@tracklang@currentmatch{\@tracklang@currentmatch 1}%
        \else
          \edef\@tracklang@currentmatch{\@tracklang@currentmatch 0}%
        \fi
        \ifx\@tracklang@currentmatch\@tracklang@fullmatch
          \let#2\@tracklang@dialect
        \else
          \ifnum\@tracklang@currentmatch>\@tracklang@bestmatch\relax
            \let\TrackedDialectClosestSubMatch\@tracklang@dialect
            \let\@tracklang@bestmatch\@tracklang@currentmatch
          \fi
        \fi
     }%
  }%
}
\def\@tracklang@fullmatch{1111}
\def\TrackLangFromEnv{%
 \def\TrackLangEnvLang{}%
 \def\TrackLangEnvTerritory{}%
 \def\TrackLangEnvCodeSet{}%
 \def\TrackLangEnvModifier{}%
  \ifx\TrackLangEnv\undefined
    \TrackLangQueryEnv
  \fi
  \ifx\TrackLangEnv\empty
     \@tracklang@warn{\string\TrackLangFromEnv\space
     non-operational as \string\TrackLangEnv\space is empty}%
  \else
    \ifx\TrackLangEnv\undefined
       \@tracklang@warn{\string\TrackLangFromEnv\space
       non-operational as \string\TrackLangEnv\space hasn't been
       defined}%
    \else
       \@tracklang@parse@track@locale{\TrackLangEnv}%
       \let\TrackLangEnvLang\@TrackLangEnvLang
       \let\TrackLangEnvTerritory\@TrackLangEnvTerritory
       \let\TrackLangEnvCodeSet\@TrackLangEnvCodeSet
       \let\TrackLangEnvModifier\@TrackLangEnvModifier
    \fi
  \fi
}
\def\TrackLocale#1{%
  \@tracklang@ifundef{@tracklang@add@#1}%
  {%
    \@tracklang@parse@track@locale{#1}%
  }%
  {%
    \@tracklang@nameuse{@tracklang@add@#1}%
  }%
}
\def\@tracklang@parse@track@locale#1{%
  \@tracklang@parse@locale{#1}%
  \@tracklang@track@locale
}
\def\@tracklang@track@locale{%
  \TrackLangIfKnownLangFromIso{\@TrackLangEnvLang}
  {%
    \edef\@tracklang@lang{\TrackLangGetKnownLangFromIso\@TrackLangEnvLang}%
    \let\@tracklang@dialect\@TrackLangEnvLang
    \ifx\@TrackLangEnvSubLang\empty
    \else
      \edef\@tracklang@dialect{\@tracklang@dialect-\@TrackLangEnvSubLang}%
    \fi
    \ifx\@TrackLangEnvScript\empty
    \else
      \edef\@tracklang@dialect{\@tracklang@dialect-\@TrackLangEnvScript}%
    \fi
    \ifx\@TrackLangEnvTerritory\empty
    \else
      \edef\@tracklang@dialect{\@tracklang@dialect-\@TrackLangEnvTerritory}%
    \fi
    \ifx\@TrackLangEnvModifier\empty
    \else
      \edef\@tracklang@dialect{\@tracklang@dialect-\@TrackLangEnvModifier}%
    \fi
    \ifx\@TrackLangEnvVariant\empty
    \else
      \edef\@tracklang@dialect{\@tracklang@dialect-\@TrackLangEnvVariant}%
    \fi
    \@tracklang@ifundef{@tracklang@add@\@tracklang@dialect}%
    {%
       \edef\@tracklang@dialect{%
         \@TrackLangEnvLang
         \@TrackLangEnvSubLang
         \@TrackLangEnvScript
         \@TrackLangEnvTerritory
         \@TrackLangEnvModifier
         \@TrackLangEnvVariant}%
       \AddTrackedDialect{\@tracklang@dialect}{\@tracklang@lang}%
       \AddTrackedLanguageIsoCodes{\@tracklang@lang}%
       \ifx\@TrackLangEnvFirstSubLang\empty
       \else
         \expandafter\AddTrackedIsoLanguage
           \expandafter\ThreeLetterExtIsoLanguageCode
           \expandafter{\@TrackLangEnvFirstSubLang}%
           {\@tracklang@dialect}%
       \fi
    }%
    {%
      \csname @tracklang@add@\@tracklang@dialect\endcsname
    }%
  }%
  {%
    \@tracklang@warn{Unknown language code `\@TrackLangEnvLang'}%
    \edef\@tracklang@dialect{%
      \@TrackLangEnvLang
      \@TrackLangEnvSubLang
      \@TrackLangEnvScript
      \@TrackLangEnvTerritory
      \@TrackLangEnvModifier
      \@TrackLangEnvVariant}%
    \AddTrackedDialect{\@tracklang@dialect}{\@TrackLangEnvLang}%
    \expandafter\@tracklang@hasthirdchar
       \@TrackLangEnvLang\relax\relax\relax\@end@tracklang@hasthirdchar
     {%
       \AddTrackedIsoLanguage{639-2}{\@TrackLangEnvLang}{\@tracklang@lang}%
     }%
     {%
         \AddTrackedIsoLanguage{639-1}{\@TrackLangEnvLang}{\@tracklang@lang}%
     }%
  }%
  \ifx\@TrackLangEnvTerritory\empty
  \else
    \AddTrackedIsoLanguage{3166-1}{\@TrackLangEnvTerritory}%
     {\@tracklang@dialect}%
  \fi
  \ifx\@TrackLangEnvModifier\empty
  \else
    \SetTrackedDialectModifier{\@tracklang@dialect}{\@TrackLangEnvModifier}%
  \fi
  \ifx\@TrackLangEnvVariant\empty
  \else
    \SetTrackedDialectVariant{\@tracklang@dialect}{\@TrackLangEnvVariant}%
  \fi
  \ifx\@TrackLangEnvScript\empty
  \else
    \SetTrackedDialectScript{\@tracklang@dialect}{\@TrackLangEnvScript}%
  \fi
  \ifx\@TrackLangEnvSubLang\empty
  \else
    \SetTrackedDialectSubLang{\@tracklang@dialect}{\@TrackLangEnvSubLang}%
  \fi
  \ifx\@TrackLangEnvAdditional\empty
  \else
    \SetTrackedDialectAdditional{\@tracklang@dialect}{\@TrackLangEnvAdditional}%
  \fi
}
\ifx\@tracklang@declareoption\undefined
  \def\@tracklang@declareoption#1{}
\fi
\def\TrackLangDeclareLanguageOption#1#2#3#4#5#6#7{%
  \@tracklang@ifundef{@tracklang@add@#1}%
  {%
    \TrackLangNewLanguage{#1}{#2}{#3}{#4}{#5}{#6}{#7}%
    \@tracklang@namedef{@tracklang@add@#1}{%
      \AddTrackedLanguage{#1}%
      \AddTrackedLanguageIsoCodes{#1}%
      \AddTrackedCountryIsoCode{#1}%
    }%
    \@tracklang@declareoption{#1}%
  }%
  {%
    \@tracklang@err{language option `#1' has already been defined}{}%
  }%
}
\TrackLangDeclareLanguageOption{abkhaz}{ab}{abk}{}{}{}{Cyrl}
\TrackLangDeclareLanguageOption{afar}{aa}{aar}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{afrikaans}{af}{afr}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{akan}{ak}{aka}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{albanian}{sq}{sqi}{alb}{}{}{Latn}
\TrackLangDeclareLanguageOption{amharic}{am}{amh}{}{}{ET}{Ethi}
\TrackLangDeclareLanguageOption{anglosaxon}{}{ang}{}{}{}{Runr}
\TrackLangDeclareLanguageOption{apache}{}{apa}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{arabic}{ar}{ara}{}{}{}{Arab}
\TrackLangDeclareLanguageOption{aragonese}{an}{arg}{}{}{ES}{Latn}
\TrackLangDeclareLanguageOption{armenian}{hy}{hye}{arm}{}{}{Armn}
\TrackLangDeclareLanguageOption{assamese}{as}{asm}{}{}{}{Beng}
\TrackLangDeclareLanguageOption{asturian}{}{ast}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{avaric}{av}{ava}{}{}{}{Cyrl}
\TrackLangDeclareLanguageOption{avestan}{ae}{ave}{}{}{}{Avst}
\TrackLangDeclareLanguageOption{aymara}{ay}{aym}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{azerbaijani}{az}{aze}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{bahasai}{id}{ind}{}{}{IN}{Latn}
\TrackLangDeclareLanguageOption{bahasam}{ms}{msa}{may}{}{MY}{Latn}
\TrackLangDeclareLanguageOption{bambara}{bm}{bam}{}{}{ML}{Latn}
\TrackLangDeclareLanguageOption{bashkir}{ba}{bak}{}{}{}{Cyrl}
\TrackLangDeclareLanguageOption{basque}{eu}{eus}{baq}{}{}{Latn}
\TrackLangDeclareLanguageOption{belarusian}{be}{bel}{}{}{}{Cyrl}
\TrackLangDeclareLanguageOption{bengali}{bn}{ben}{}{}{}{Beng}
\TrackLangDeclareLanguageOption{berber}{}{ber}{}{}{}{}
\TrackLangDeclareLanguageOption{bihari}{bh}{bih}{}{}{}{}
\TrackLangDeclareLanguageOption{bislama}{bi}{bis}{}{}{VU}{Latn}
\TrackLangDeclareLanguageOption{bokmal}{nb}{nob}{}{}{NO}{Latn}
\TrackLangDeclareLanguageOption{bosnian}{bs}{bos}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{breton}{br}{bre}{}{}{FR}{Latn}
\TrackLangDeclareLanguageOption{bulgarian}{bg}{bul}{}{}{}{Cyrl}
\TrackLangDeclareLanguageOption{burmese}{my}{mya}{bur}{}{}{Mymr}
\TrackLangDeclareLanguageOption{catalan}{ca}{cat}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{chamorro}{ch}{cha}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{chechen}{ce}{che}{}{}{}{Cyrl}
\TrackLangDeclareLanguageOption{chichewa}{ny}{nya}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{chinese}{zh}{zho}{chi}{}{}{Hans}
\TrackLangDeclareLanguageOption{churchslavonic}{cu}{chu}{}{}{}{Glag}
\TrackLangDeclareLanguageOption{chuvash}{cv}{chv}{}{}{RU}{Cyrl}
\TrackLangDeclareLanguageOption{coptic}{}{cop}{}{}{}{Copt}
\TrackLangDeclareLanguageOption{cornish}{kw}{cor}{}{}{GB}{Latn}
\TrackLangDeclareLanguageOption{corsican}{co}{cos}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{cree}{cr}{cre}{}{}{}{Cans}
\TrackLangDeclareLanguageOption{croatian}{hr}{hrv}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{czech}{cs}{ces}{cze}{}{}{Latn}
\TrackLangDeclareLanguageOption{danish}{da}{dan}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{divehi}{dv}{div}{}{}{MV}{Thaa}
\TrackLangDeclareLanguageOption{dutch}{nl}{nld}{dut}{}{}{Latn}
\TrackLangDeclareLanguageOption{dzongkha}{dz}{dzo}{}{}{BT}{Tibt}
\TrackLangDeclareLanguageOption{easternpunjabi}{pa}{pan}{}{}{IN}{Guru}
\TrackLangDeclareLanguageOption{english}{en}{eng}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{esperanto}{eo}{epo}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{estonian}{et}{est}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{ewe}{ee}{ewe}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{faroese}{fo}{fao}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{farsi}{fa}{fas}{per}{}{}{Arab}
\TrackLangDeclareLanguageOption{fijian}{fj}{fij}{}{}{FJ}{Latn}
\TrackLangDeclareLanguageOption{finnish}{fi}{fin}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{french}{fr}{fra}{fre}{}{}{Latn}
\TrackLangDeclareLanguageOption{friulan}{}{fur}{}{}{IT}{Latn}
\TrackLangDeclareLanguageOption{fula}{ff}{ful}{}{}{}{}
\TrackLangDeclareLanguageOption{galician}{gl}{glg}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{ganda}{lg}{lug}{}{}{UG}{Latn}
\TrackLangDeclareLanguageOption{georgian}{ka}{kat}{geo}{}{}{Geor}
\TrackLangDeclareLanguageOption{german}{de}{deu}{ger}{}{}{Latn}
\TrackLangDeclareLanguageOption{greek}{el}{ell}{gre}{}{}{Grek}
\TrackLangDeclareLanguageOption{guarani}{gn}{grn}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{gujarati}{gu}{guj}{}{}{}{Gujr}
\TrackLangDeclareLanguageOption{haitian}{ht}{hat}{}{}{HT}{Latn}
\TrackLangDeclareLanguageOption{hausa}{ha}{hau}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{hebrew}{he}{heb}{}{}{}{Hebr}
\TrackLangDeclareLanguageOption{herero}{hz}{her}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{hindi}{hi}{hin}{}{}{}{Deva}
\TrackLangDeclareLanguageOption{hirimotu}{ho}{hmo}{}{}{PG}{Latn}
\TrackLangDeclareLanguageOption{icelandic}{is}{isl}{ice}{}{IS}{Latn}
\TrackLangDeclareLanguageOption{ido}{io}{ido}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{igbo}{ig}{ibo}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{interlingua}{ia}{ina}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{interlingue}{ie}{ile}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{inuktitut}{iu}{iku}{}{}{}{Cans}
\TrackLangDeclareLanguageOption{inupiaq}{ik}{ipk}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{irish}{ga}{gle}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{italian}{it}{ita}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{japanese}{ja}{jpn}{}{}{}{Hani}
\TrackLangDeclareLanguageOption{javanese}{jv}{jav}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{kalaallisut}{kl}{kal}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{kannada}{kn}{kan}{}{}{IN}{Knda}
\TrackLangDeclareLanguageOption{kanuri}{kr}{kau}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{kashmiri}{ks}{kas}{}{}{IN}{}
\TrackLangDeclareLanguageOption{kazakh}{kk}{kaz}{}{}{}{}
\TrackLangDeclareLanguageOption{khmer}{km}{khm}{}{}{}{Khmr}
\TrackLangDeclareLanguageOption{kikuyu}{ki}{kik}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{kinyarwanda}{rw}{kin}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{kirundi}{rn}{run}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{komi}{kv}{kom}{}{}{RU}{Cyrl}
\TrackLangDeclareLanguageOption{kongo}{kg}{kon}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{korean}{ko}{kor}{}{}{}{Hang}
\TrackLangDeclareLanguageOption{kurdish}{ku}{kur}{}{}{}{}
\TrackLangDeclareLanguageOption{kwanyama}{kj}{kua}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{kyrgyz}{ky}{kir}{}{}{}{Cyrl}
\TrackLangDeclareLanguageOption{lao}{lo}{lao}{}{}{}{Laoo}
\TrackLangDeclareLanguageOption{latin}{la}{lat}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{latvian}{lv}{lav}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{limburgish}{li}{lim}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{lingala}{ln}{lin}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{lithuanian}{lt}{lit}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{lsorbian}{}{dsb}{}{}{DE}{Latn}
\TrackLangDeclareLanguageOption{lubakatanga}{lu}{lub}{}{}{CD}{Latn}
\TrackLangDeclareLanguageOption{luxembourgish}{lb}{ltz}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{macedonian}{mk}{mkd}{mac}{}{}{Cyrl}
\TrackLangDeclareLanguageOption{magyar}{hu}{hun}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{malagasy}{mg}{mlg}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{malayalam}{ml}{mal}{}{}{IN}{Mlym}
\TrackLangDeclareLanguageOption{maltese}{mt}{mlt}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{manx}{gv}{glv}{}{}{IM}{Latn}
\TrackLangDeclareLanguageOption{maori}{mi}{mri}{mao}{}{NZ}{Latn}
\TrackLangDeclareLanguageOption{marathi}{mr}{mar}{}{}{IN}{Deva}
\TrackLangDeclareLanguageOption{marshallese}{mh}{mah}{}{}{MH}{Latn}
\TrackLangDeclareLanguageOption{mongolian}{mn}{mon}{}{}{}{Mong}
\TrackLangDeclareLanguageOption{nauruan}{na}{nau}{}{}{NR}{Latn}
\TrackLangDeclareLanguageOption{navajo}{nv}{nav}{}{}{US}{Latn}
\TrackLangDeclareLanguageOption{ndonga}{ng}{ndo}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{nepali}{ne}{nep}{}{}{}{Deva}
\TrackLangDeclareLanguageOption{nko}{}{nqo}{}{}{}{Nkoo}
\TrackLangDeclareLanguageOption{northernndebele}{nd}{nde}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{nynorsk}{nn}{nno}{}{}{NO}{Latn}
\TrackLangDeclareLanguageOption{norsk}{no}{nor}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{northernsotho}{}{nso}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{nuosu}{ii}{iii}{}{}{CN}{Yiii}
\TrackLangDeclareLanguageOption{occitan}{oc}{oci}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{ojibwe}{oj}{oji}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{oromo}{om}{orm}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{oriya}{or}{ori}{}{}{}{Orya}
\TrackLangDeclareLanguageOption{ossetian}{os}{oss}{}{}{}{Cyrl}
\TrackLangDeclareLanguageOption{pali}{pi}{pli}{}{}{}{Brah}
\TrackLangDeclareLanguageOption{pashto}{ps}{pus}{}{}{}{Arab}
\TrackLangDeclareLanguageOption{piedmontese}{}{}{}{pms}{IT}{Latn}
\TrackLangDeclareLanguageOption{polish}{pl}{pol}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{portuges}{pt}{por}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{quechua}{qu}{que}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{romanian}{ro}{ron}{rum}{}{}{Latn}
\TrackLangDeclareLanguageOption{romansh}{rm}{roh}{}{}{CH}{Latn}
\TrackLangDeclareLanguageOption{russian}{ru}{rus}{}{}{}{Cyrl}
\TrackLangDeclareLanguageOption{samin}{se}{sme}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{sanskrit}{sa}{san}{}{}{}{}
\TrackLangDeclareLanguageOption{samoan}{sm}{smo}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{sango}{sg}{sag}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{sardinian}{sc}{srd}{}{}{IT}{Latn}
\TrackLangDeclareLanguageOption{scottish}{gd}{gla}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{serbian}{sr}{srp}{}{}{}{Cyrl}
\TrackLangDeclareLanguageOption{shona}{sn}{sna}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{sindhi}{sd}{snd}{}{}{}{Sind}
\TrackLangDeclareLanguageOption{sinhalese}{si}{sin}{}{}{LK}{Sinh}
\TrackLangDeclareLanguageOption{slovak}{sk}{slk}{slo}{}{}{Latn}
\TrackLangDeclareLanguageOption{slovene}{sl}{slv}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{somali}{so}{som}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{southernndebele}{nr}{nbl}{}{}{ZA}{Latn}
\TrackLangDeclareLanguageOption{southernsotho}{st}{sot}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{spanish}{es}{spa}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{sudanese}{su}{sun}{}{}{}{Sund}
\TrackLangDeclareLanguageOption{swahili}{sw}{swa}{}{}{}{}
\TrackLangDeclareLanguageOption{swati}{ss}{ssw}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{swedish}{sv}{swe}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{syriac}{}{syr}{}{}{}{Syrc}
\TrackLangDeclareLanguageOption{tagalog}{tl}{tgl}{}{}{PH}{Latn}
\TrackLangDeclareLanguageOption{tahitian}{ty}{tah}{}{}{PF}{Latn}
\TrackLangDeclareLanguageOption{tai}{}{tai}{}{}{}{}
\TrackLangDeclareLanguageOption{tajik}{tg}{tgk}{}{}{}{Cyrl}
\TrackLangDeclareLanguageOption{tamil}{ta}{tam}{}{}{}{Taml}
\TrackLangDeclareLanguageOption{tatar}{tt}{tat}{}{}{}{Cyrl}
\TrackLangDeclareLanguageOption{telugu}{te}{tel}{}{}{IN}{Telu}
\TrackLangDeclareLanguageOption{thai}{th}{tha}{}{}{TH}{Thai}
\TrackLangDeclareLanguageOption{tibetan}{bo}{bod}{tib}{}{}{Tibt}
\TrackLangDeclareLanguageOption{tigrinya}{ti}{tir}{}{}{}{Ethi}
\TrackLangDeclareLanguageOption{tonga}{to}{ton}{}{}{TO}{Latn}
\TrackLangDeclareLanguageOption{tsonga}{ts}{tso}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{tswana}{tn}{tsn}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{turkish}{tr}{tur}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{turkmen}{tk}{tuk}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{twi}{tw}{twi}{}{}{GH}{Latn}
\TrackLangDeclareLanguageOption{ukrainian}{uk}{ukr}{}{}{UA}{Cyrl}
\TrackLangDeclareLanguageOption{urdu}{ur}{urd}{}{}{}{Arab}
\TrackLangDeclareLanguageOption{usorbian}{}{hsb}{}{}{DE}{Latn}
\TrackLangDeclareLanguageOption{uyghur}{ug}{uig}{}{}{CN}{Arab}
\TrackLangDeclareLanguageOption{uzbek}{uz}{uzb}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{venda}{ve}{ven}{}{}{ZA}{Latn}
\TrackLangDeclareLanguageOption{vietnamese}{vi}{vie}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{volapuk}{vo}{vol}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{walloon}{wa}{wln}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{welsh}{cy}{cym}{wel}{}{}{Latn}
\TrackLangDeclareLanguageOption{westernfrisian}{fy}{fry}{}{}{NL}{Latn}
\TrackLangDeclareLanguageOption{wolof}{wo}{wol}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{xhosa}{xh}{xho}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{yiddish}{yi}{yid}{}{}{}{Hebr}
\TrackLangDeclareLanguageOption{yoruba}{yo}{yor}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{zhuang}{za}{zha}{}{}{CN}{Hani}
\TrackLangDeclareLanguageOption{zulu}{zu}{zul}{}{}{}{Latn}
\def\TrackLangDeclareDialectOption#1#2#3#4#5#6#7{%
  \@tracklang@ifundef{@tracklang@add@#1}%
  {%
    \ifx\relax#3\relax
     \ifx\relax#4\relax
      \ifx\relax#5\relax
        \@tracklang@namedef{@tracklang@add@#1}{%
          \AddTrackedDialect{#1}{#2}%
          \AddTrackedLanguageIsoCodes{#2}%
          \def\@tracklang@dialect{#1}%
        }%
      \else
        \@tracklang@namedef{@tracklang@add@#1}{%
          \AddTrackedDialect{#1}{#2}%
          \AddTrackedLanguageIsoCodes{#2}%
          \SetTrackedDialectVariant{#1}{#5}%
          \def\@tracklang@dialect{#1}%
        }%
      \fi
     \else
       \ifx\relax#5\relax
         \@tracklang@namedef{@tracklang@add@#1}{%
           \AddTrackedDialect{#1}{#2}%
           \AddTrackedLanguageIsoCodes{#2}%
           \SetTrackedDialectModifier{#1}{#4}%
           \def\@tracklang@dialect{#1}%
         }%
       \else
         \@tracklang@namedef{@tracklang@add@#1}{%
           \AddTrackedDialect{#1}{#2}%
           \AddTrackedLanguageIsoCodes{#2}%
           \SetTrackedDialectModifier{#1}{#4}%
           \SetTrackedDialectVariant{#1}{#5}%
           \def\@tracklang@dialect{#1}%
         }%
       \fi
     \fi
    \else
     \ifx\relax#4\relax
       \ifx\relax#5\relax
          \@tracklang@namedef{@tracklang@add@#1}{%
            \AddTrackedDialect{#1}{#2}%
            \AddTrackedLanguageIsoCodes{#2}%
            \AddTrackedIsoLanguage{3166-1}{#3}{#1}%
            \def\@tracklang@dialect{#1}%
          }%
       \else
          \@tracklang@namedef{@tracklang@add@#1}{%
            \AddTrackedDialect{#1}{#2}%
            \AddTrackedLanguageIsoCodes{#2}%
            \AddTrackedIsoLanguage{3166-1}{#3}{#1}%
            \SetTrackedDialectVariant{#1}{#5}%
            \def\@tracklang@dialect{#1}%
          }%
       \fi
     \else
       \ifx\relax#5\relax
          \@tracklang@namedef{@tracklang@add@#1}{%
            \AddTrackedDialect{#1}{#2}%
            \AddTrackedLanguageIsoCodes{#2}%
            \AddTrackedIsoLanguage{3166-1}{#3}{#1}%
            \SetTrackedDialectModifier{#1}{#4}%
            \def\@tracklang@dialect{#1}%
          }%
       \else
          \@tracklang@namedef{@tracklang@add@#1}{%
            \AddTrackedDialect{#1}{#2}%
            \AddTrackedLanguageIsoCodes{#2}%
            \AddTrackedIsoLanguage{3166-1}{#3}{#1}%
            \SetTrackedDialectModifier{#1}{#4}%
            \SetTrackedDialectVariant{#1}{#5}%
            \def\@tracklang@dialect{#1}%
          }%
       \fi
     \fi
    \fi
    \ifx\relax#6\relax
    \else
      \expandafter
       \let\expandafter\@tracklang@tmp\csname @tracklang@add@#1\endcsname
      \expandafter\def\csname @tracklang@add@#1\expandafter\endcsname
        \expandafter{\@tracklang@tmp\SetTrackedDialectLabelMap{#1}{#6}}%
    \fi
    \ifx\relax#7\relax
    \else
      \expandafter
       \let\expandafter\@tracklang@tmp\csname @tracklang@add@#1\endcsname
      \expandafter\def\csname @tracklang@add@#1\expandafter\endcsname
        \expandafter{\@tracklang@tmp\SetTrackedDialectScript{#1}{#7}}%
    \fi
    \@tracklang@declareoption{#1}%
  }%
  {%
    \@tracklang@err{dialect option `#1' has already been defined}{}%
  }%
}
\TrackLangDeclareDialectOption{acadian}{french}{}{}{}{}{}
\TrackLangDeclareDialectOption{american}{english}{US}{}{}{}{}
\TrackLangDeclareDialectOption{australian}{english}{AU}{}{}{}{}
\TrackLangDeclareDialectOption{austrian}{german}{AT}{}{}{}{}
\TrackLangDeclareDialectOption{naustrian}{german}{AT}{new}{1996}{}{}
\TrackLangDeclareDialectOption{bahasa}{bahasai}{IN}{}{}{}{}
\TrackLangDeclareDialectOption{brazil}{portuges}{BR}{}{}{}{}
\TrackLangDeclareDialectOption{brazilian}{portuges}{BR}{}{}{}{}
\TrackLangDeclareDialectOption{british}{english}{GB}{}{}{}{}
\TrackLangDeclareDialectOption{canadian}{english}{CA}{}{}{}{}
\TrackLangDeclareDialectOption{canadien}{french}{CA}{}{}{}{}
\TrackLangDeclareDialectOption{croatia}{croatian}{HR}{}{}{}{}
\TrackLangDeclareDialectOption{istriacountycroatian}{croatian}{HR}{}{}{}{}
\TrackLangDeclareDialectOption{istriacountyitalian}{italian}{HR}{}{}{}{}
\TrackLangDeclareDialectOption{netherlands}{dutch}{NL}{}{}{}{}
\TrackLangDeclareDialectOption{persian}{farsi}{}{}{}{}{}
\TrackLangDeclareDialectOption{flemish}{dutch}{BE}{}{}{}{}
\TrackLangDeclareDialectOption{francais}{french}{}{}{}{}{}
\TrackLangDeclareDialectOption{frenchb}{french}{}{}{}{}{}
\TrackLangDeclareDialectOption{france}{french}{FR}{}{}{}{}
\TrackLangDeclareDialectOption{belgique}{french}{BE}{}{}{}{}
\TrackLangDeclareDialectOption{belgiangerman}{german}{BE}{}{}{}{}
\TrackLangDeclareDialectOption{nbelgiangerman}{german}{BE}{new}{1996}{ngerman}{}
\TrackLangDeclareDialectOption{friulian}{friulan}{IT}{}{}{}{}
\TrackLangDeclareDialectOption{friulano}{friulan}{IT}{}{}{}{}
\TrackLangDeclareDialectOption{furlan}{friulan}{IT}{}{}{}{}
\TrackLangDeclareDialectOption{kurmanji}{kurdish}{}{}{}{}{}
\TrackLangDeclareDialectOption{galicien}{galician}{}{}{}{}{}
\TrackLangDeclareDialectOption{deutsch}{german}{}{}{}{}{}
\TrackLangDeclareDialectOption{ngerman}{german}{}{new}{1996}{}{}
\TrackLangDeclareDialectOption{ngermanb}{german}{}{new}{1996}{ngerman}{}
\TrackLangDeclareDialectOption{germanb}{german}{}{}{}{}{}
\TrackLangDeclareDialectOption{ngermanDE}{german}{DE}{new}{1996}{ngerman}{}
\TrackLangDeclareDialectOption{germanDE}{german}{DE}{}{}{}{}
\TrackLangDeclareDialectOption{hungarian}{magyar}{HU}{}{}{}{}
\TrackLangDeclareDialectOption{indon}{bahasai}{IN}{}{}{}{}
\TrackLangDeclareDialectOption{indonesian}{bahasai}{IN}{}{}{}{}
\TrackLangDeclareDialectOption{gaeilge}{irish}{}{}{}{}{}
\TrackLangDeclareDialectOption{IEirish}{irish}{IE}{}{}{}{}
\TrackLangDeclareDialectOption{GBirish}{irish}{GB}{}{}{}{}
\TrackLangDeclareDialectOption{IEenglish}{english}{IE}{}{}{british}{}
\TrackLangDeclareDialectOption{italy}{italian}{IT}{}{}{}{}
\TrackLangDeclareDialectOption{vatican}{italian}{VA}{}{}{}{}
\TrackLangDeclareDialectOption{sanmarino}{italian}{SM}{}{}{}{}
\TrackLangDeclareDialectOption{sloveneistriaitalian}{italian}{SI}{}{}{}{}
\TrackLangDeclareDialectOption{jerseyenglish}{english}{JE}{}{}{british}{}
\TrackLangDeclareDialectOption{jerseyfrench}{french}{JE}{}{}{}{}
\TrackLangDeclareDialectOption{guernseyenglish}{english}{GG}{}{}{british}{}
\TrackLangDeclareDialectOption{guernseyfrench}{french}{GG}{}{}{}{}
\TrackLangDeclareDialectOption{latein}{latin}{}{}{}{}{}
\TrackLangDeclareDialectOption{lowersorbian}{lsorbian}{DE}{}{}{}{}
\TrackLangDeclareDialectOption{malay}{bahasam}{MY}{}{}{}{}
\TrackLangDeclareDialectOption{meyalu}{bahasam}{MY}{}{}{}{}
\TrackLangDeclareDialectOption{maltamaltese}{maltese}{MT}{}{}{}{}
\TrackLangDeclareDialectOption{maltaenglish}{english}{MT}{}{}{british}{}
\TrackLangDeclareDialectOption{newzealand}{english}{NZ}{}{}{}{}
\TrackLangDeclareDialectOption{isleofmanenglish}{english}{IM}{}{}{british}{}
\TrackLangDeclareDialectOption{norwegian}{norsk}{NO}{}{}{}{}
\TrackLangDeclareDialectOption{piemonteis}{piedmontese}{IT}{}{}{}{}
\TrackLangDeclareDialectOption{polutonikogreek}{greek}{}{polyton}{}{}{}
\TrackLangDeclareDialectOption{polutoniko}{greek}{}{polyton}{}{}{}
\TrackLangDeclareDialectOption{portuguese}{portuges}{}{}{}{}{}
\TrackLangDeclareDialectOption{portugal}{portuges}{PT}{}{}{}{}
\TrackLangDeclareDialectOption{romansch}{romansh}{}{}{}{}{}
\TrackLangDeclareDialectOption{rumantsch}{romansh}{}{}{}{}{}
\TrackLangDeclareDialectOption{romanche}{romansh}{}{}{}{}{}
\TrackLangDeclareDialectOption{russianb}{russian}{}{}{}{}{}
\TrackLangDeclareDialectOption{gaelic}{scottish}{}{}{}{}{}
\TrackLangDeclareDialectOption{GBscottish}{scottish}{GB}{}{}{}{}
\TrackLangDeclareDialectOption{serbianc}{serbian}{}{}{}{}{Cyrl}
\TrackLangDeclareDialectOption{serbianl}{serbian}{}{}{}{}{Latn}
\TrackLangDeclareDialectOption{slovenian}{slovene}{}{}{}{}{}
\TrackLangDeclareDialectOption{slovenia}{slovene}{SI}{}{}{slovenian}{}
\TrackLangDeclareDialectOption{sloveneistriaslovenian}{slovene}{SI}{}{}{slovenian}{}
\TrackLangDeclareDialectOption{spainspanish}{spanish}{ES}{}{}{}{}
\TrackLangDeclareDialectOption{argentinespanish}{spanish}{AR}{}{}{}{}
\TrackLangDeclareDialectOption{bolivianspanish}{spanish}{BO}{}{}{}{}
\TrackLangDeclareDialectOption{chilianspanish}{spanish}{CL}{}{}{}{}
\TrackLangDeclareDialectOption{columbianspanish}{spanish}{CO}{}{}{}{}
\TrackLangDeclareDialectOption{costaricanspanish}{spanish}{CR}{}{}{}{}
\TrackLangDeclareDialectOption{cubanspanish}{spanish}{CU}{}{}{}{}
\TrackLangDeclareDialectOption{dominicanspanish}{spanish}{DO}{}{}{}{}
\TrackLangDeclareDialectOption{ecudorianspanish}{spanish}{EC}{}{}{}{}
\TrackLangDeclareDialectOption{elsalvadorspanish}{spanish}{SV}{}{}{}{}
\TrackLangDeclareDialectOption{guatemalanspanish}{spanish}{GT}{}{}{}{}
\TrackLangDeclareDialectOption{honduranspanish}{spanish}{HN}{}{}{}{}
\TrackLangDeclareDialectOption{mexicanspanish}{spanish}{MX}{}{}{}{}
\TrackLangDeclareDialectOption{nicaraguanspanish}{spanish}{NI}{}{}{}{}
\TrackLangDeclareDialectOption{panamaspanish}{spanish}{PA}{}{}{}{}
\TrackLangDeclareDialectOption{paraguayspanish}{spanish}{PY}{}{}{}{}
\TrackLangDeclareDialectOption{peruvianspanish}{spanish}{PE}{}{}{}{}
\TrackLangDeclareDialectOption{puertoricospanish}{spanish}{PR}{}{}{}{}
\TrackLangDeclareDialectOption{uruguayspanish}{spanish}{UY}{}{}{}{}
\TrackLangDeclareDialectOption{venezuelanspanish}{spanish}{VE}{}{}{}{}
\TrackLangDeclareDialectOption{swissgerman}{german}{CH}{}{}{}{}
\TrackLangDeclareDialectOption{nswissgerman}{german}{CH}{new}{1996}{ngerman}{}
\TrackLangDeclareDialectOption{swissfrench}{french}{CH}{}{}{}{}
\TrackLangDeclareDialectOption{swissitalian}{italian}{CH}{}{}{}{}
\TrackLangDeclareDialectOption{swissromansh}{romansh}{CH}{}{}{}{}
\TrackLangDeclareDialectOption{UKenglish}{english}{GB}{}{}{}{}
\TrackLangDeclareDialectOption{ukraineb}{ukrainian}{UA}{}{}{}{}
\TrackLangDeclareDialectOption{ukraine}{ukrainian}{UA}{}{}{}{}
\TrackLangDeclareDialectOption{uppersorbian}{usorbian}{DE}{}{}{}{}
\TrackLangDeclareDialectOption{USenglish}{english}{US}{}{}{}{}
\TrackLangDeclareDialectOption{valencian}{catalan}{}{}{}{}{}
\TrackLangDeclareDialectOption{valencien}{catalan}{}{}{}{}{}
\TrackLangDeclareDialectOption{cymraeg}{welsh}{}{}{}{}{}
\TrackLangDeclareDialectOption{GBwelsh}{welsh}{GB}{}{}{}{}
\def\LetTrackLangSynonym#1#2{%
  \expandafter\let\csname @tracklang@add@#1\expandafter\endcsname
    \csname @tracklang@add@#2\endcsname
}
\def\LetTrackLangOption#1#2{%
  \LetTrackLangSynonym{#1}{#2}%
  \@tracklang@declareoption{#1}%
}
\LetTrackLangOption{en-US}{american}
\LetTrackLangOption{en-GB}{british}
\LetTrackLangOption{en-AU}{australian}
\LetTrackLangOption{en-NZ}{newzealand}
\LetTrackLangOption{en-CA}{canadian}
\LetTrackLangOption{fr-CA}{canadien}
\LetTrackLangOption{fr-BE}{belgique}
\LetTrackLangOption{pt-BR}{brazilian}
\LetTrackLangOption{it-HR}{istriacountyitalian}
\LetTrackLangOption{nl-BE}{flemish}
\LetTrackLangOption{fr-FR}{france}
\LetTrackLangOption{de-DE}{germanDE}
\LetTrackLangOption{de-BE}{belgiangerman}
\LetTrackLangOption{en-GG}{guernseyenglish}
\LetTrackLangOption{fr-GG}{guernseyfrench}
\LetTrackLangOption{it-IT}{italy}
\LetTrackLangOption{mt-MT}{maltamaltese}
\LetTrackLangOption{en-MT}{maltaenglish}
\LetTrackLangOption{en-IM}{isleofmanenglish}
\LetTrackLangOption{en-JE}{jerseyenglish}
\LetTrackLangOption{fr-JE}{jerseyfrench}
\LetTrackLangOption{nl-NL}{netherlands}
\LetTrackLangOption{pt-PT}{portugal}
\LetTrackLangOption{it-SM}{sanmarino}
\LetTrackLangOption{sl-SI}{slovenia}
\LetTrackLangOption{it-SI}{sloveneistriaitalian}
\LetTrackLangOption{es-ES}{spainspanish}
\LetTrackLangOption{es-AR}{argentinespanish}
\LetTrackLangOption{es-BO}{bolivianspanish}
\LetTrackLangOption{es-CL}{chilianspanish}
\LetTrackLangOption{es-CO}{columbianspanish}
\LetTrackLangOption{es-CR}{costaricanspanish}
\LetTrackLangOption{es-CU}{cubanspanish}
\LetTrackLangOption{es-DO}{dominicanspanish}
\LetTrackLangOption{es-EC}{ecudorianspanish}
\LetTrackLangOption{es-SV}{elsalvadorspanish}
\LetTrackLangOption{es-GT}{guatemalanspanish}
\LetTrackLangOption{es-HN}{honduranspanish}
\LetTrackLangOption{es-MX}{mexicanspanish}
\LetTrackLangOption{es-NI}{nicaraguanspanish}
\LetTrackLangOption{es-PA}{panamaspanish}
\LetTrackLangOption{es-PY}{paraguayspanish}
\LetTrackLangOption{es-PE}{peruvianspanish}
\LetTrackLangOption{es-PR}{puertoricospanish}
\LetTrackLangOption{es-UY}{uruguayspanish}
\LetTrackLangOption{es-VE}{venezuelanspanish}
\LetTrackLangOption{de-CH}{swissgerman}
\LetTrackLangOption{fr-CH}{swissfrench}
\LetTrackLangOption{it-CH}{swissitalian}
\LetTrackLangOption{rm-CH}{swissromansh}
\LetTrackLangOption{it-VA}{vatican}
\LetTrackLangOption{ga-IE}{IEirish}
\LetTrackLangOption{ga-GB}{GBirish}
\LetTrackLangOption{en-IE}{IEenglish}
\LetTrackLangOption{de-AT-1996}{naustrian}
\LetTrackLangOption{de-AT}{austrian}
\LetTrackLangOption{id-IN}{bahasa}
\LetTrackLangOption{ms-MY}{malay}
\LetTrackLangOption{hr-HR}{croatia}
\LetTrackLangOption{de-DE-1996}{ngermanDE}
\LetTrackLangOption{de-CH-1996}{nswissgerman}
\LetTrackLangOption{hu-HU}{hungarian}
\LetTrackLangOption{gd-GB}{GBscottish}
\LetTrackLangOption{cy-GB}{GBwelsh}
\long\def\IfTrackedLanguage#1#2#3{%
  \edef\@tracklang@element{#1}%
  \ifx\@tracklang@element\empty
    #3%
  \else
    \expandafter\@tracklang@ifinlist\expandafter{\@tracklang@element}%
      \@tracklang@languages
    {%
      #2%
    }%
    {%
      #3%
    }%
  \fi
}
\long\def\IfTrackedDialect#1#2#3{%
  \@tracklang@ifundef{@tracklang@fromdialect@#1}{#3}{#2}%
}
\long\def\IfTrackedIsoCode#1#2#3#4{%
  \@tracklang@ifundef{@tracklang@#1@isotolang@#2}{#4}{#3}%
}
\long\def\IfTrackedLanguageHasIsoCode#1#2#3#4{%
  \@tracklang@ifundef{@tracklang@#1@isofromlang@#2}{#4}{#3}%
}
\long\def\ForEachTrackedLanguage#1#2{%
  \@tracklang@for#1:=\@tracklang@languages\do{#2}%
}
\long\def\ForEachTrackedDialect#1#2{%
  \@tracklang@for#1:=\@tracklang@dialects\do{#2}%
}
\long\def\AnyTrackedLanguages#1#2{%
  \ifx\@tracklang@languages\empty
    #2%
  \else
    #1%
  \fi
}
\long\def\IfTrackedLanguageFileExists#1#2#3#4#5{%
   \def\CurrentTrackedTag{}%
   \SetCurrentTrackedDialect{#1}%
   \IfTrackedDialect{#1}%
   {%
     \edef\CurrentTrackedTag{#1}%
     \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}%
     {#4}%
     {%
       \IfTrackedLanguageHasIsoCode
         {639-1}{\CurrentTrackedLanguage}
       {%
          \edef\CurrentTrackedIsoCode{%
             \TrackedIsoCodeFromLanguage
               {639-1}{\CurrentTrackedLanguage}}%
          \ifx\CurrentTrackedRegion\empty
            \let\CurrentTrackedTag\CurrentTrackedIsoCode
            \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}%
            {#4}
            {%
              \IfTrackedLanguageHasIsoCode
                {639-2}{\CurrentTrackedLanguage}
              {%
                 \edef\CurrentTrackedIsoCode{%
                    \TrackedIsoCodeFromLanguage
                      {639-2}{\CurrentTrackedLanguage}}%
                 \let\CurrentTrackedTag\CurrentTrackedIsoCode
                 \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}%
                 {#4}%
                 {%
                   \let\CurrentTrackedTag\CurrentTrackedLanguage
                   \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}{#4}{#5}%
                 }%
              }%
              {%
               \let\CurrentTrackedTag\CurrentTrackedLanguage
               \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}{#4}{#5}%
              }%
            }%
          \else
            \edef\CurrentTrackedTag{%
              \CurrentTrackedIsoCode-\CurrentTrackedRegion}%
            \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}%
            {#4}
            {%
              \IfTrackedLanguageHasIsoCode
              {639-2}{\CurrentTrackedLanguage}
              {%
                \let\org@currenttrackedisocode\CurrentTrackedIsoCode
                \edef\CurrentTrackedIsoCode{%
                  \TrackedIsoCodeFromLanguage
                  {639-2}{\CurrentTrackedLanguage}}%
                \edef\CurrentTrackedTag{%
                  \CurrentTrackedIsoCode-\CurrentTrackedRegion}%
                \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}%
                {#4}%
                {%
                  \let\CurrentTrackedTag\org@currenttrackedisocode
                  \let\org@currenttrackedisocode\CurrentTrackedIsoCode
                  \let\CurrentTrackedIsoCode\CurrentTrackedTag
                  \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}%
                  {#4}
                  {%
                    \let\CurrentTrackedIsoCode\org@currenttrackedisocode
                    \let\CurrentTrackedTag\CurrentTrackedIsoCode
                    \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}%
                    {#4}%
                    {%
                      \let\CurrentTrackedTag\CurrentTrackedRegion
                      \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}%
                      {#4}%
                      {%
                        \let\CurrentTrackedTag\CurrentTrackedLanguage
                        \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}{#4}{#5}%
                      }%
                    }%
                  }%
                }%
              }%
              {%
                \let\CurrentTrackedTag\CurrentTrackedIsoCode
                \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}%
                {#4}%
                {%
                  \let\CurrentTrackedTag\CurrentTrackedRegion
                  \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}%
                  {#4}%
                  {%
                    \let\CurrentTrackedTag\CurrentTrackedLanguage
                    \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}{#4}{#5}%
                  }%
                }%
              }%
            }%
          \fi
       }%
       {%
         \IfTrackedLanguageHasIsoCode
           {639-2}{\CurrentTrackedLanguage}
         {%
            \edef\CurrentTrackedIsoCode{%
               \TrackedIsoCodeFromLanguage
               {639-2}{\CurrentTrackedLanguage}}%
         }%
         {%
           \IfTrackedLanguageHasIsoCode
             {639-3}{\CurrentTrackedLanguage}
           {%
              \edef\CurrentTrackedIsoCode{%
                 \TrackedIsoCodeFromLanguage
                 {639-3}{\CurrentTrackedLanguage}}%
           }%
           {%
              \let\CurrentTrackedIsoCode\empty
           }%
         }%
         \ifx\CurrentTrackedIsoCode\empty
           \ifx\CurrentTrackedRegion\empty
             \let\CurrentTrackedTag\CurrentTrackedLanguage
             \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}{#4}{#5}%
           \else
             \let\CurrentTrackedTag\CurrentTrackedRegion
             \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}%
             {#4}%
             {%
               \let\CurrentTrackedTag\CurrentTrackedLanguage
               \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}{#4}{#5}%
             }%
           \fi
         \else
            \ifx\CurrentTrackedRegion\empty
              \let\CurrentTrackedTag\CurrentTrackedIsoCode
              \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}%
              {#4}%
              {%
                \let\CurrentTrackedTag\CurrentTrackedLanguage
                \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}{#4}{#5}%
              }%
            \else
              \edef\CurrentTrackedTag{%
                \CurrentTrackedIsoCode-\CurrentTrackedRegion}%
              \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}%
              {#4}%
              {%
                \let\CurrentTrackedTag\CurrentTrackedIsoCode
                \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}%
                {#4}%
                {%
                  \let\CurrentTrackedTag\CurrentTrackedRegion
                  \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}%
                  {#4}%
                  {%
                    \let\CurrentTrackedTag\CurrentTrackedLanguage
                    \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}{#4}{#5}%
                  }%
                }%
              }%
            \fi
         \fi
       }%
     }%
   }%
   {#5}% unknown dialect
}
\ifx\ProvidesFile\undefined
  \long\def\TrackLangProvidesResource#1#2{%
    \ifx\TrackLangRequireDialectPrefix\undefined
      \@tracklang@err{Resources files using
        \string\TrackLangProvidesResource\space
        must be loaded with \string\TrackLangRequireDialect}%
    \fi
    \ifx#2[\relax
      \def\@tracklang@next{%
        \@tracklang@providesresource{\TrackLangRequireDialectPrefix-#1.ldf}#2%
      }
    \else
      \expandafter\xdef\csname ver@\TrackLangRequireDialectPrefix
        -#1.ldf\endcsname{}%
      {%
        \newlinechar=`\^^J
        \def\MessageBreak{^^J}%
        \message{^^JFile: \TrackLangRequireDialectPrefix-#1.ldf^^J}%
      }%
      \long\def\@tracklang@next{#2}%
    \fi
    \@tracklang@next
  }
  \def\@tracklang@providesresource#1[#2]{%
    \expandafter\xdef\csname ver@#1\endcsname{#2}%
     {%
       \newlinechar=`\^^J
       \def\MessageBreak{^^J}%
       \message{^^JFile: #1 #2^^J}%
     }%
  }
\else
  \def\TrackLangProvidesResource#1{%
    \ifx\TrackLangRequireDialectPrefix\undefined
      \@tracklang@err{Resources files using
        \string\TrackLangProvidesResource\space
        must be loaded with \string\TrackLangRequireDialect}%
    \fi
    \ProvidesFile{\TrackLangRequireDialectPrefix-#1.ldf}%
  }
\fi
\def\TrackLangAddToHook{\noop@TrackLangAddToHook}
\def\noop@TrackLangAddToHook#1#2{%
  \@tracklang@err{\string\TrackLangAddToHook\space
  only permitted within resource files}
}
\def\@TrackLangAddToHook#1#2{%
  \@tracklang@ifundef{#2\CurrentTrackedDialect}%
  {%
    \IfTrackedDialectHasMapping{\CurrentTrackedDialect}%
    {%
      \edef\@tracklang@tmp{%
        \csname @tracklang@dialectmap@tohook@\CurrentTrackedDialect\endcsname}%
      \@tracklang@ifundef{#2\@tracklang@tmp}%
      {%
        \@tracklang@ifundef{#2\CurrentTrackedLanguage}%
        {%
          #1%
        }%
        {%
          \@tracklang@addtohook{#2}{\CurrentTrackedLanguage}{#1}%
        }%
      }%
      {%
        \@tracklang@addtohook{#2}{\@tracklang@tmp}{#1}%
      }%
    }%
    {%
      \@tracklang@ifundef{#2\CurrentTrackedLanguage}%
      {%
      }%
      {%
        \@tracklang@addtohook{#2}{\CurrentTrackedLanguage}{#1}%
      }%
    }%
  }%
  {%
     \@tracklang@addtohook{#2}{\CurrentTrackedDialect}{#1}%
  }%
  #1%
}
\def\@tracklang@addtohook#1#2#3{%
 \expandafter\let\expandafter\@tracklang@hook\csname #1#2\endcsname
 \expandafter
  \gdef\csname#1#2\expandafter\endcsname\expandafter{\@tracklang@hook#3}%
}
\def\TrackLangAddToCaptions#1{\TrackLangAddToHook{#1}{captions}}
\def\SetTrackedDialectLabelMap#1#2{%
  \@tracklang@enamedef{@tracklang@dialectmap@tohook@#1}{#2}%
  \@tracklang@enamedef{@tracklang@dialectmap@fromhook@#2}{#1}%
}
\def\IfTrackedDialectHasMapping#1#2#3{%
  \@tracklang@ifundef{@tracklang@dialectmap@tohook@#1}{#3}{#2}%
}
\def\IfHookHasMappingFromTrackedDialect#1#2#3{%
  \@tracklang@ifundef{@tracklang@dialectmap@fromhook@#1}{#3}{#2}%
}
\def\GetTrackedDialectToMapping#1{%
  \@tracklang@ifundef{@tracklang@dialectmap@tohook@#1}{#1}%
  {\csname @tracklang@dialectmap@tohook@#1\endcsname}%
}
\def\GetTrackedDialectFromMapping#1{%
  \@tracklang@ifundef{@tracklang@dialectmap@fromhook@#1}{#1}%
  {\csname @tracklang@dialectmap@fromhook@#1\endcsname}%
}
\def\TrackLangRequireResource{\noop@TrackLangRequireResource}
\def\noop@TrackLangRequireResource#1{%
  \@tracklang@err{\string\TrackLangRequireResource\space
  only permitted within resource files}
}
\def\@TrackLangRequireResource#1{%
  \@tracklang@ifundef{ver@\TrackLangRequireDialectPrefix-#1.ldf}%
  {%
    \@tracklang@IfFileExists{\TrackLangRequireDialectPrefix-#1.ldf}%
    {%
      \input \TrackLangRequireDialectPrefix-#1.ldf
    }%
    {%
      \@tracklang@warn{No `\TrackLangRequireDialectPrefix' support for
      language/region `#1'\MessageBreak
      (resource file `\TrackLangRequireDialectPrefix-#1.ldf' not found)}%
    }%
  }%
  {}%
}
\def\TrackLangRequireResourceOrDo{%
  \noop@TrackLangRequireResourceOrDo
}
\def\noop@TrackLangRequireResourceOrDo#1#2#3{%
  \@tracklang@err{\string\TrackLangRequireResourceOrDo\space
  only permitted within resource files}
}
\def\@TrackLangRequireResourceOrDo#1#2#3{%
  \@tracklang@ifundef{ver@\TrackLangRequireDialectPrefix-#1.ldf}%
  {%
    \@tracklang@IfFileExists{\TrackLangRequireDialectPrefix-#1.ldf}%
    {%
      \input \TrackLangRequireDialectPrefix-#1.ldf
      #2%
    }%
    {%
      \@tracklang@warn{No `\TrackLangRequireDialectPrefix' support for
      language/region `#1'\MessageBreak
      (resource file `\TrackLangRequireDialectPrefix-#1.ldf' not found)}%
    }%
  }%
  {#3}%
}
\def\TrackLangRequestResource{\noop@TrackLangRequestResource}
\def\noop@TrackLangRequestResource#1#2{%
  \@tracklang@err{\string\TrackLangRequestResource\space
  only permitted within resource files}
}
\def\@TrackLangRequestResource#1#2{%
  \@tracklang@ifundef{ver@\TrackLangRequireDialectPrefix-#1.ldf}%
  {%
    \@tracklang@IfFileExists{\TrackLangRequireDialectPrefix-#1.ldf}%
    {%
      \input \TrackLangRequireDialectPrefix-#1.ldf
    }%
    {#2}%
  }%
  {}%
}
\def\TrackLangRequireDialect{\@TrackLangRequireDialect}
\def\noop@TrackLangRequireDialect#1{%
  \ifx[#1\relax
    \def\@tracklang@next{\@noop@TrackLangRequireDialect[}%
  \else
    \def\@tracklang@next{\@noop@TrackLangRequireDialect[]{#1}}%
  \fi
  \@tracklang@next
}
\def\@noop@TrackLangRequireDialect[#1]#2#3{%
  \@tracklang@err{\string\TrackLangRequireDialect\space
  only permitted within resource files}
}
\def\@TrackLangRequireDialect#1{%
  \ifx[#1\relax
    \def\@tracklang@next{\@@TrackLangRequireDialect[}%
  \else
    \def\@tracklang@next{%
      \@@TrackLangRequireDialect
        [\TrackLangRequireResource{\CurrentTrackedTag}]{#1}}%
  \fi
  \@tracklang@next
}
\def\@@TrackLangRequireDialect[#1]#2#3{%
   \def\TrackLangRequireDialectPrefix{#2}%
   \IfTrackedLanguageFileExists{#3}%
   {#2-}% prefix
   {.ldf}% suffix
   {%
     \let\TrackLangRequireResource\@TrackLangRequireResource
     \let\TrackLangRequireResourceOrDo\@TrackLangRequireResourceOrDo
     \let\TrackLangRequestResource\@TrackLangRequestResource
     \let\TrackLangRequireDialect\noop@TrackLangRequireDialect
     \let\TrackLangAddToHook\@TrackLangAddToHook
     #1%
     \let\TrackLangRequireResource\noop@TrackLangRequireResource
     \let\TrackLangRequireResourceOrDo\noop@TrackLangRequireResourceOrDo
     \let\TrackLangRequestResource\noop@TrackLangRequestResource
     \let\TrackLangRequireDialect\@TrackLangRequireDialect
     \let\TrackLangAddToHook\noop@TrackLangAddToHook
   }%
   {%
     \@tracklang@warn{No `#2' support for dialect `#3'}%
   }%
}
\@tracklang@restore@at
\endinput
%%
%% End of file `tracklang.tex'.

